Pull Request Decision Explained: An Empirical Overview

Context: Pull-based development model is widely used in open source, leading the trends in distributed software development. One aspect which has garnered significant attention is studies on pull request decision - identifying factors for explanation. Objective: This study builds on a decade long research on pull request decision to explain it. We empirically investigate how factors influence pull request decision and scenarios that change the influence of factors. Method: We identify factors influencing pull request decision on GitHub through a systematic literature review and infer it by mining archival data. We collect a total of 3,347,937 pull requests with 95 features from 11,230 diverse projects on GitHub. Using this data, we explore the relations of the factors to each other and build mixed-effect logistic regression models to empirically explain pull request decision. Results: Our study shows that a small number of factors explain pull request decision with the integrator same or different from the submitter as the most important factor. We also noted that some factors are important only in special cases e.g., the percentage of failed builds is important for pull request decision when continuous integration is used.

==> experiment.tex <==
\section{Experiment}
\label{Experiment}
We firstly build up base models using popular factors occur in previous studies. Then based on the base model, we analysis the influence of different kinds of factors, including comment related factors, CI related factors.

\subsection{Data Preperation}
Based on Zhang et al.~\cite{msr2020_ours}, we extend the data according to Session~\ref{session:slr} and get 110 factors in the end.
In order to have enough data for better analyze. We use the \emph{country\_code} column in users table of GHTorrent, and use pycountry~\footnote{https://pypi.org/project/pycountry/} to generate the country name of users and fill in the empty values. The number of records with non empty values for \texttt{contrib\_country}, \texttt{inte\_country} and \texttt{same\_country} increase 546,682, 747,204 and 796,083 respectively.
We removed the pull requests with negative values of factor \texttt{ci\_latency}, \texttt{first\_response\_time}, \texttt{account\_creation\_days} and \texttt{project\_age} according to the technical report~\footnote{https://github.com/zhangxunhui/new\_pullreq\_msr2020/blob/master/technical\_report.pdf}, and we get 3,281,386 results in the end.

% \subsection{Factor Selection}
% There are 100+ factors in our dataset, in order to make a big picture of pull-based development, we firstly select the factors that have a strong correlation with the decision and latency of pull request.

% Firstly, We select those factors that have at least 1 study considered that it is significantly important. For decision making of pull request, we get 50 factors. For pull request latency, we get XX factors.
% Then we remove those strongly correlated factors according to the correlation between each pair of factors. For correlation between continuous factors, we use Spearman coefficient to measure the correlation (strong correlation > 0.7). For correlation between categorical variables, we use Cramer's V value (strong correlation > 0.5). For correlation between continuous and categorical factors, we use Eta-Squared value (strong correlation > 0.14).

%% I changed the factors selection part by calculating the occur times of each factor in previous studies

\subsection{Base Model Creation}
We firstly select the popular factors which appear frequently in previous studies using the following steps:

\begin{enumerate}
    \item Calculate the number of papers that each factor appear in previous studies.
    \item Select the factors that appear more than 2 times (75th percentile of boxplot equals 2), and 20 factors left.
    \item Remove strongly correlated factors. If two factors are strongly correlated, we keep the one that appears more in previous studies. However, if they appear the same number of times, we manually decide which one to keep (we choose \texttt{ci\_exists} instead of \texttt{ci\_test\_passed}, because for base model, we want firstly know whether pull request uses CI or not). To measure the correlation between each pair of factors, we use Spearman correlation coefficient ($\rho$) to measure correlation between continuous factors, Cramér's V ($\Phi_c$) for categorical factors and partial Eta-squared ($\eta^2$) for correlation between continuous and categorical factors. We treat $\rho>0.7$~\cite{Gousios_exploratory}, $\Phi_c>\frac{0.5}{df}$~\cite{cohen_1969} and $\eta^2>0.14$~\cite{cohen_1969} as strong correlations.
\end{enumerate}

After the above steps, 16 factors left. Based on these factors, we build up mixed-effect logistic regression model with project id as random effect.

==> methods.tex <==
%%% 针对每个RQ，介绍研究方法
\section{Study Design}
\label{methods}

% Describe the 
\subsection{Methods}
In this part, we will explain the research methods used in this paper, including the basic methods and the approaches for each research question.
Also, we will describe the dataset and the methods used for data processing.
In order to build the big picture of both the decision making and latency of pull requests, we use the regression models, which can not only explain the importance of factors, but also present the detailed influence direction.

\subsubsection{Regression Model}
Here, we create mixed effects logistic regression models with project identifier as the random effect and all the measured factors as fixed effects.
A major advantage of mixed effect model is that it can eliminate the correlated observations within a subject~\cite{linear_mixed_effect}. Here, pull requests for the same project tend to have similar behavior.
We use the \emph{glmer} function of \emph{lme4}~\cite{R_lme4} package in R to fit models for the acceptance of pull request.

For the latency of pull request, we build up linear mixed-effect model using \emph{lmerTest}~\cite{R_lmertest} package in R according to previous studies~\cite{Yu_wait, Yu_determinants}. 
Similarly, we treat project identifier as random effect and all the measured factors as fixed effects.

\subsubsection{Evaluation Metrics}
In order to evaluate the effectiveness of model and the importance of factors, we compare models' predictive performance with random predictors and calculate factors' relative importance in a unified dimension.

% \textbf{Goodness of Fit:}
% For both decision making and latency related models, we present 5 values, including 
% Log Likelihood~\cite{fisher_stats}, which represents the log value of the likelihood of fitting the training dataset,
% Akaike Information Criterion (AIC)~\cite{AIC} and Bayesian Information Criterion (BIC)~\cite{BIC}, which are both maximum likelihood estimate driven and penalize free parameters in an effort to combat overfitting, but in different ways.
% Deviance~\cite{glm}, which measures the deviance of the fitted logistic model with respect to a perfect model.
% For AIC, BIC, Deviance, the smaller their values, the stronger is the fit of the model.
% For Log Likelihood, it's the opposite.
% Since the decision making models are classification models, so we also use metric Area Under Curve (AUC)~\cite{AUC}, which indicates model's capability of distinguishing between classes.
% For AUC value, it is considered acceptable if greater than 0.5~\cite{Rastogi_relationshipESEM}.

\textbf{Predictive Performance:}
In order to explain the predictive performance of related models, we split the pull requests according to the close time, and use 90\% of prior pull requests for training and the last 10\% for testing.

For the decision making of pull request, we build up a random decision making classifier as the baseline, which randomly predicts whether a pull request can be merged according to the merge rate in training dataset.
Then use weighted precision, weighted recall, weighted f-score and AUC value\cite{Bradley_AUC} to measure the predictive performance of both baseline model and logistic regression model, as the data is highly imbalanced in our dataset.

For the latency of pull request, we also build up random predictor as the baseline, which randomly select values between the minimum and maximum pull request lifetime in training set.
Then we use 2 standard metrics to compare the performance of the regression model and the baseline model, namely MAE (Mean Absolute Error)\cite{Willmott_MAE} and MSE (Mean Square Error)\cite{Allen_MSE}.

\textbf{Relative Importance:}
In previous studies, there are several ways to measure the relative importance of predictors in linear regression and logistic regression models.

For latency related models, previous studies used the``dispersion importance''~\cite{Chao_relative_importance, Thomas_relative_importance}, which is measured by the proportion of variance explained by each predictor to describe the relative importance.
Therefore, we also inherit this method, and calculate the proportion of sum of square of each factor.
Here, we use Type II anova function in package \emph{lmerTest}~\cite{R_lmertest} of R language, as we are building models on imbalanced data~\cite{Langsrud_anova}.

For decision making related models, since the response variable is a categorical variable, we use the standardized regression coefficient~\cite{standardized_coefficients}, which is one of the most common approaches~\cite{relative_importance} to measure the relative importance of each factor in logistic regression model.
We can use the absolute value of the standardized coefficient to represent the relative importance of predictors.

In order to compare the difference of the factor importance in different models, we use the importance ranking and compare the ranking change.

\subsubsection{Approaches for Each Research Question}
\label{methods_each_RQ}
In this part, we will explain the approaches used in each research question.

\textbf{RQ1}, we first do a systematic literature review (SLR) of previous studies which focused on analyzing the related factors of the acceptance and latency of pull-based development.
By following the guidelines of Keele et al.~\cite{Keele_slr_guideline}, we define the following steps: 1) define the research questions of SLR; 2) Define the search strategy, including keywords, combined search string and online libraries; 3) Define the inclusion and exclusion of publication criteria; 4) Extra data from the paper to answer the research questions.
By extracting all the quantitative factors, the related significance and influence direction, we can have an overall perspective of previous studies.

\textbf{RQ2}, based on our previous work~\cite{msr2020_ours}, we expand the data collection of related factors.
Then we build up mixed effect logistic regression models for the decision making and mixed effect linear regression models for the latency of pull request using data after August 2013 in order to compare with previous study~\cite{Gousios_exploratory}.
Here, we build up the \textbf{basic models} for
the decision making and latency of pull request using factors that are not dependent on other factors, as shown in Table\ref{factor_dependent_table}, we remove the factors in the left column because they are meaningful only when the dependent factors on the right have special values,
\emph{e.g.} for factor \emph{perc\_pos\_emotion} and \emph{perc\_neg\_emotion}, they only make sense when there exist comments (\emph{has\_comments}=1), otherwise the values are empty.

\textbf{RQ3}, we split the dataset according to different contexts, including both pull request level and project level to see the change of factors' relative importance.
For pull request level contexts, in order to explain the factors not considered in \textbf{RQ2}, we build up \textbf{special case models} according to Table \ref{factor_dependent_table}, including pull requests that have comments (\emph{has\_comments}=1), pull requests that have contributor's comment (\emph{contrib\_comment}=1), pull request that have integrator's comment (\emph{inte\_comment}=1), pull requests that are not contributed and integrated by the same user (\emph{same\_user=0}) and pull requests that use CI tools (\emph{ci\_exists}=1).
Also, in order to check the influence of factors in different time periods, we split the pull request according to the close time.
For project level contexts, we divide the projects in different ways, \emph{e.g.} team size at data collection time.
%Here we use the Spearman's rank correlation~\cite{spearman_rank_correlation} to represent the change of the importance ranking of factors comparing to those in the \textbf{basic models}.

\subsubsection{Approaches for Data Processing}
\label{method_data_processing}
In this part, we will describe the methods that we use to do data processing.

\textbf{Standardization:} Before building up models, all factors are centered and scaled using \emph{scale} function in R language in order to normalize all the factors into the same scale.

\textbf{Correlation:} In order to measure the correlation between each pair of factors, we use Spearman correlation coefficient ($\rho$) for continuous factors, Cramér's V ($\Phi_c$) for categorical factors and partial Eta-squared ($\eta^2$) for correlation between continuous and categorical factors. We treat $\rho>0.7$~\cite{Gousios_exploratory}, $\Phi_c>\frac{0.5}{df}$~\cite{cohen_1969} and $\eta^2>0.14$~\cite{cohen_1969} as strong correlations.
The strongly correlated factors and the selected factor of each group can be seen in Table~\ref{strongly_correlated_factors}.
The reasons for the selection can be seen in Section \ref{model_building}.

\textbf{Collinearity:} For the collinearity problem, except for removing the strongly correlated factors,
we also calculate the VIF value for each factor in regression models using \emph{vif} function of \emph{car} package in R language, and make sure that all the values are less than 5~\cite{cohen_applied}.


\subsection{Dataset}
In this paper, we used the dataset proposed in our previous study~\cite{msr2020_ours}, where the factors are divided into 3 categories, including developer related, project related and pull request related factors.
The description of the factors can be seen in Table~\ref{factor_descriptive_statistics}.
\input{tables/dataset_description}
After doing systematic literature review (see Section~\ref{session:slr}), we expand the dataset with factors which can be seen in Table~\ref{factor_descriptive_statistics} marked by $\oplus$.

\subsubsection{Data Preprocessing}
\begin{enumerate}
\item In order to have enough data for better analysis.
We use the \emph{country\_code} column in users table of GHTorrent~\cite{gousios_ghtorrent}, and use package \emph{pycountry}~\footnote{https://pypi.org/project/pycountry/} to generate the country name of users and fill in the empty values. The number of records with non empty values for \emph{contrib\_country}, \emph{inte\_country} and \emph{same\_country} increase 546,682, 747,204 and 796,083 respectively. The expanded country information can be seen on Github~\footnote{https://github.com/zhangxunhui/TSE\_pull-based-development/blob/master/country\_info.csv}.

\item To reduce the impact of special cases,
we remove the pull requests with negative values of factor \emph{ci\_latency}, \emph{first\_response\_time}, \emph{account\_creation\_days} and \emph{project\_age} according to the technical report~\footnote{https://github.com/zhangxunhui/new\_pullreq\_msr2020/blob/master/ technical\_report.pdf}.
% 3,281,386 left
There are also some pull requests that have 0 commits when creating the pull request, which means that they created a draft pull request first, then make commits.
% 3,219,729
After all the operations, we get 3,194,607 pull requests in the end.

\item We remove factor \emph{bug\_fix} because there lacks of valid values (99.3\% empty values), and add a new factor called \emph{same\_user} because some factors including \emph{same\_country}, \emph{same\_affiliation} and personality difference related factors (\emph{e.g. open\_diff}) only make sense when the contributor and integrator are not the same user. And we find that 43.6\% pull requests are integrated by the contributor. So adding this factor is also very important.

\item We standardize all the predictors by adding the value ‘one’ to continuous factors and log-transform the result to stabilize the variance and then use the \emph{scale} function in R language to scale all the predictors into one scale with mean value 0 and standard deviation 1.\footnote{https://medium.com/@sjacks/feature-transformation-21282d1a3215}

\item For the response factor of latency related models (\emph{lifetime\_minutes}), we also do the log-transformation, which can not only pull outlying data from a positively skewed distribution closer to the bulk of the data, but also improve the interpretability.
Then the exponent of coefficient can be explained as a "unit" increase in predictor causes 1\% increase or decrease in average (geometric) pull request latency~\footnote{https://towardsdatascience.com/interpreting-the-coefficients-of-linear-regression-cc31d4c6f235}.
However, for the response factor of decision making related models (\emph{merged\_or\_not}), as it is a binary factor, we do not do any transformation.
And the absolute value of odds ratio can be explained as "the increase or decrease of the odds of acceptance occurring per 'unit' of the factor".
Here, a 'unit' of each factor is one standard deviation from the standardization of log-transformed for continuous factors or one standard deviation from the standardization for categorical factors.
\end{enumerate}

\subsubsection{Model Building}
\label{model_building}
\begin{enumerate}
    \item After calculating the correlation between each pair of factors, we remove those strongly correlated ones (following the criteria in Section~\ref{method_data_processing}), as shown in Table~\ref{strongly_correlated_factors}.
    There are different reasons for the choice of factors, including
    \textbf{Previous Study:} in previous studies, they also chose in the same way, \emph{e.g.} Gousios et al.~\cite{Gousios_exploratory} chose \emph{test\_lines\_per\_kloc} rather than \emph{test\_cases\_per\_kloc} and \emph{asserts\_per\_kloc}.
    \textbf{Occur Times:} calculate how many times did factors appear in related works and keep the most frequent factor (\emph{e.g.} comparing to \emph{perc\_external\_contribs}, \emph{social\_strength} and \emph{requester\_succ\_rate}, \emph{core\_member} occurs most often).
    \textbf{Significance:} if some factors occur the same times in previous studies, we tend to select the one whose influence significance is measured in previous study (\emph{e.g.} factor \emph{sloc} was marked as significantly influencing the decision making, however the significance of factor \emph{language} is unknown. In this way, we can compare our result with previous studies).
    \textbf{Representative:} comparing to other factors in the set, we can find one of them is more representative (\emph{e.g.} factor \emph{has\_comments} can represent more information, and after there exists comment, we can discuss the influence of \emph{core\_comment}, \emph{contrib\_comment}, \emph{inte\_comment} and \emph{has\_exchange}).
    \textbf{Missing Value:} some factors have lots of missing values, so we choose the one with more non-empty values (\emph{e.g.} factor \emph{open\_issue\_num} has more non-empty values than \emph{inte\_affiliation}).
    \textbf{Discussion:} for some strongly correlated groups, we decide to choose one of the factors through discussion.
    For factor \emph{perc\_neg\_emotion}, comparing to \emph{perc\_contrib\_neg\_emo}, \emph{contrib\_first\_emo} and \emph{inte\_first\_emo}, it can more effectively reflect the overall emotional tendency of the review process.
    Similarly, we choose factor \emph{perc\_pos\_emotion} rather than \emph{inte\_first\_emo}, \emph{perc\_inte\_neg\_emo} rather than \emph{inte\_first\_emo}, \emph{perc\_inte\_pos\_emo} rather than \emph{inte\_first\_emo} and \emph{perc\_contrib\_pos\_emo} rather than \emph{contrib\_first\_emo}.
    For factor \emph{same\_country}, it considers both the geographical location of contributor and integrator and also the relation between them, so we keep it instead of \emph{contrib\_country}.
    Similarly, we choose factor \emph{same\_affiliation} rather than \emph{contrib\_affiliation}.
    For factor \emph{same\_user}, we decide to keep it instead of others because it is related to some special cases as shown in Table \ref{factor_dependent_table}).
    
    
    \item In order to build models without multicollinearity problem, we check the models' VIF value to make sure that all the factors' VIF value is less than 5. Therefore, we remove factor \emph{num\_code\_comments}, which is also moderately correlated with factor \emph{num\_comments} ($\rho=0.63$).
    \item When building models for \textbf{RQ2}, we filter those factors that only make sense conditionally (\emph{e.g.} if the contributor and integrator is the same user, the personality difference like openness difference does not make sense).
    Therefore, when building models, we firstly use the pre-conditional factors (right column in Table~\ref{factor_dependent_table}) and ignore those dependent factors (left column in Table~\ref{factor_dependent_table}), we call the built models \textbf{basic models}.
    Then we discuss the dependent factors with certain pre-conditions (only in this way, we can clearly know the actual influence of some dependent variables in special circumstances), and we call these built models \textbf{special case models}.
    For the decision making of pull request, after removing dependent factors, 46 factors left (marked by $\dagger$ in Table~\ref{factor_descriptive_statistics}). 
    \item For the latency of pull request, we change factor \emph{lifetime\_minutes} to the dependent factor, and remove pull requests that were reopened, same as what Yue et al. did in their previous work~\cite{Yu_determinants, Yu_wait}. Thereafter, 44 factors left for analysis (marked by $\ddagger$ in Table~\ref{factor_descriptive_statistics}).
\end{enumerate}
\input{tables/correlation_table}
\input{tables/factor_dependent_table}

==> slr.tex <==
\section{Systematic Literature Review}
\label{session:slr}

Historically, research investigating the factors associated with pull-based development has focused on the decision making and latency of pull request.
Therefore, in order to answer \textbf{RQ1}, have a broad perspective of all the related previous studies and clearly understand how different factors influence the acceptance and latency of pull request,
we perform a systematic literature review following the guidelines of kitchenham et al.~\cite{kitchenham_slr}.

\subsection{Literature Reivew Question}

We come up with the following questions for the literature review part, which are the sub-RQs of \textbf{RQ1}:

\emph{RQ1-1: What factors influence the acceptance and latency of pull request?}

\emph{RQ1-2: What's the influence direction and significance of each factor?}


\subsection{Search Strategy}
\label{search_strategy}

Firstly, after discussing with all the authors of this paper, the defined search keywords including "pull based" and "pull request".
    
Secondly, we combine all the research keywords using \emph{OR} logic, and the search string is shown as follows:
    
(\emph{"pull based" OR "pull request"})
    
Thirdly, we select the following online libraries and search engines, which are widely used by software engineering researchers, including \emph{Google Scholar}, \emph{ACM Digital Library}, \emph{IEEExplore}, \emph{Web of Science} and \emph{EI Compendex}.
By searching the Boolean string in different databases, we get 3,941 papers in total (\emph{Google Scholar}: 1,000; \emph{ACM Digital Library}: 1,433; \emph{IEEExplore}: 352; \emph{Web of Science}: 487 and \emph{EI Compendex}: 669). (The query is conducted on 2020-04-17).
    
Finally, because the limitation of 1,000 return results of \emph{Google Scholar}. We conduct another round of search only for the year 2020 so that we can make sure all the related papers are included after doing snowballing(see Section \ref{snowballing}).
Thereafter, we get 1,610 papers for \emph{Google Scholar}, and 4,551 in total in the end.


\subsection{Inclusion/Exclusion Criteria}
\label{inclusion_exclusion_criteria}

In order to filter those unrelated papers, we define several criteria.

Firstly, We remove the duplicated paper by title automatically, and 3,255 papers left.

Secondly, we manually check the titles of remained papers, and classify them into different groups.
\begin{enumerate}
    \item Papers that are not written in English (45 excluded).
    \item Duplicate papers that are not checked out automatically (115 excluded).
    \item Papers that have corresponding extended ones (12 excluded).
    \item Papers that are not related to the acceptance or latency of pull request according to the title (2,810 excluded).
    \item Papers that are related to pull-based development study, which have direct keywords in title (34 included).
    \item Papers that are not sure if they are related to pull-based development, which is related to open source software development but no keywords about pull-based development (239 included).
\end{enumerate}

Thirdly, we combine the papers in Group 5) and 6) in the second step, and manually check the abstract. We get 51 papers that are related to our research field in the end. But not all of them directly focus on analyzing the factors that influence the decision making or latency of pull request. Therefore, we classify the related papers into two sub-groups according to their research goals.
\begin{enumerate}
    \item Directly related papers: the goal of the paper is about the decision making or latency of pull request (33 papers).
    \item Indirectly related papers: the goal of the paper is not about the pull request decision making or latency, but just have some related results (18 papers).
\end{enumerate}
Here, the division of directly related and indirect related papers is just for the follow-up snowballing process.
Our goal isn't identifying all the indirectly related papers.

\subsection{Snowballing}
\label{snowballing}
To prevent the missing of related papers, we manually check the reference list of all the 33 directly related papers in Section~\ref{inclusion_exclusion_criteria}.

In the first round of snowballing, we get 44 papers that can be related according to the title, which are not considered in previously collected papers.
Then by reading the abstract of these papers, we get 8 related papers, of which 5 are directly related, and 3 are indirectly related. In the second round, we pick out those 5 directly related papers in the first round and repeat the previous operations. However, no more related papers can be found.
All in all, we got 59 related papers (38 directly related papers and 21 indirectly related papers).

\subsection{Data Extraction}

In this part, we extract information from these papers, including the factors mentioned, the influence direction and significance of each factor. By reading through these papers, we found that several papers and factors needs to be excluded.

\begin{enumerate}
    \item Papers that are not actually related to the study of pull request acceptance or latency when looking through the content (10). For example, paper~\cite{Bird_detecting} just present a method for identifying the submission and acceptance of patches, but not studying the acceptance or latency related factors. However, both the title and abstract have keywords "patch" and "acceptance".
    
    \item As our work mainly focus on the pull-based development on Github, some works should be excluded as not all of their measurements are applicable on Github (5). For example, Jeong et al.~\cite{Jeong_improving} built up models for predicting the acceptance of patches of Firefox and Mozilla Core projects. However, the factors like "bug severity" and "bug priority" are not applicable on Github as there is no mechanism to measure them.
    
    \item Some studies' experiments are hard to re-do (4). For example, Ford et al.~\cite{Ford_eye} used medical equipment to measure the eye track of reviewers.
    
    \item Some studies only focus on a specific range of projects, which make some of their factors hard to expand beyond the scope (4). For example, Pooput et al.~\cite{Pooput_rejection} collected the labels of Ansible community, however different communities have different labels on Github.
    
    \item There are some factors that are measured in different ways in different studies (3). For the emotion of pull request comments, Sapkota et al.~\cite{Sapkota_trust} proposed a method for estimating the trustworthiness between developers which is actually based on comment emotion. Also Ortu et al.~\cite{Ortu_mergedIssue} measured emotions using two different metrics: Valence, Arousal, Dominance and direct emotions (Joy, Love, Sadness and Anger). However, the emotion can be divided into three types according to the polarity~\cite{Iyer_master}. Therefore, we can just use the polarity to represent the comment emotion of pull requests. Calefato et al.~\cite{Calefato_trust_2017} measured the integrator's propensity to trust, however it is actually a subset of agreeableness of the big five personality traits. Iyer et al.~\cite{Iyer_tse} also measured the personality of contributor. Therefore, we measured the agreeableness instead of the subset.
    
    \item Several factors are removed because they are difficult to re-collect or not specific. For example, "project fit" (whether the pull request is in line with the goal of the target project)~\cite{Gousios_integrator}. Also, for "locality" (the file location modified in the pull request)~\cite{Soares_rejection}, it is hard to re-collect as different projects have different file locations.
\end{enumerate}

After removing the above papers, we got 32 papers left. The extracted data can be seen in Table~\ref{factor_table}, which answers the literature review questions \emph{RQ1-1} and \emph{RQ1-2}.

\begin{tcolorbox}
    Factors in previous studies mainly involve 3 aspects, namely project characteristics, developer characteristics and pull request characteristics. For developer characteristics, factors can be divided into contributor related factors, integrator related factors and the factors that marks the relationship between developers or between developer and the target project.
    Different contexts will lead to different influence direction and significance of the same factor.
\end{tcolorbox}

==> tables/dataset_description_original.tex <==
%!TEX root = ../main.tex
\begin{table*}[htbp]
\centering
\scriptsize
\caption{A comprehensive list of factors known to influence pull request decision on Github}
\label{factor_descriptive_statistics}
\begin{tabular}{| p{2.8cm} | p{5cm} | p{3.8cm} | p{5cm} |}
\toprule
Feature & Description & Feature & Description \\  \hline
\multicolumn{4}{|c|}{\textit{\textbf{Developer Characteristics}}}  \\ \hline
first\_pr $\dagger$ $\ddagger$ & Whether it is the first pull request of a contributor & prior\_review\_num $\dagger$ $\ddagger$ & The number of prior reviews of an integrator\\
core\_member $\dagger$ $\ddagger$  & Whether the contributor is a core member or not &first\_response\_time & The time interval in minutes from pull request creation to the first response by a reviewer\\
contrib\_gender $\dagger$ $\ddagger$ & The gender of a contributor & contrib\_country & Country of residence of contributor\\
same\_country &Whether contributor and integrator come from the same country & prior\_interaction & Number of times that the contributor interacted with the project in the last three months \\
same\_affiliation & Whether the contributor and the integrator belong to the same affiliation & contrib/inte\_affiliation & The affiliation that the contributor/integrator belongs to\\
contrib/inte\_X $\dagger$ $\ddagger$ & The Big Five personality traits of contributor/integrator (open: openness; cons: conscientious; extra: extraversion; agree: agreeableness; neur: neuroticism) & perc\_contrib/inte\_X\_emo & Percentage of contributor/integrator's emotion in comments (neg: negative/pos: positive) \\
X\_diff & The absolute difference of Big Five personality traits between contributor and integrator & contrib/inte\_first\_emo& The emotion of the contributor/integrator's first comment \\
social\_strength & The fraction of team members that interacted with the contributor in the last three months & contrib\_follow\_integrator & Whether the contributor follows the integrator when submitting a pull request\\ 
followers $\dagger$ $\ddagger$ & Number of followers for contributor at pull request creation time & same\_user $\dagger$ $\ddagger$ & Whether the contributor and integrator are the same user \\
prev\_pullreqs $\dagger$ $\ddagger$ & Number of pull requests submitted by a specific developer, prior to the examined pull request & account\_creation\_days $\dagger$ $\ddagger$ & The time interval in days from the contributor's account creation to the pull request creation \\
contrib\_rate\_author $\oplus$ & Percentage of contributors' commits before & & \\
\hline
\multicolumn{4}{|c|}{\textit{\textbf{Project Characteristics}}}\\ \hline
sloc $\dagger$ $\ddagger$ & Executable lines of code at pull request close time & team\_size $\dagger$ $\ddagger$ & Number of active core team members during the last 3 months prior to the pull request creation \\
language  & Programming language of project & open\_issue\_num $\dagger$ $\ddagger$ & Number of opened issues when submitting the pull request\\
project\_age $\dagger$ $\ddagger$ & Time interval in months from the project creation to the pull request creation & open\_pr\_num $\dagger$ $\ddagger$ & Number of opened pull requests when submitting the pull request\\
pushed\_delta $\dagger$ $\ddagger$ & The time interval in seconds between the opening time of the two latest pull requests & fork\_num & Number of forks of project when submitting the pull request\\ 
pr\_succ\_rate $\dagger$ $\ddagger$ & Acceptance rate of pull requests in the project & test\_lines\_per\_kloc $\dagger$ $\ddagger$ & Number of lines of test code per 1k lines of code \\ 

stars $\dagger$ $\ddagger$ & Number of stars of the project at the time of pull request creation & integrator\_availability $\dagger$ $\ddagger$ $\oplus$ & The minimum number of hours until either of the top two integrators (by number of pull-requests handled the last three months) are active \\
text\_cases\_per\_kloc & Number of test cases per 1k lines of code & asserts\_per\_kloc & Number of assertions per 1k lines of code \\
perc\_external\_contribs & Percentage of external pull request contributions & requester\_succ\_rate & Percentage of contributor's pull requests that have been merged up to the creation of the examined pull request \\
\hline
\multicolumn{4}{|c|}{\textit{\textbf{Pull Request Characteristics}}}  \\ \hline
churn\_addition & Number of added lines of code & churn\_deletion& Number of deleted lines of code \\
bug\_fix & Whether pull request fixes a bug & description\_length $\dagger$ $\ddagger$ & Word count of pull request description\\
test\_inclusion $\dagger$ $\ddagger$ & Whether test cases exists in a pull request & comment\_conflict $\dagger$ $\ddagger$ & Whether the keyword "conflict" exists in comments\\
hash\_tag $\dagger$ $\ddagger$  & Whether \# tag exists in comments or description & num\_participants & Number of participants in pull request comments \\
lifetime\_minutes $\dagger$ & Time interval in minutes from the pull request creation to the last close time & part\_num\_code & Number of participants in both pull request comment and commit comment \\
ci\_exists $\dagger$ $\ddagger$ & Whether a pull request uses continuous integration tools & ci\_build\_num & Number of CI builds\\
ci\_latency & Time interval in minutes from pull request creation to the first build finish time of CI tools & perc\_neg\_emotion & Percentage of negative emotion in comments\\
num\_code\_comments $\oplus$ & Number of code comments & perc\_pos\_emotion & Percentage of positive emotion in comments \\
test\_churn $\dagger$ $\ddagger$ & Number of lines of test code changed (added + deleted) by the pull request & num\_code\_comments\_con $\oplus$ & Number of code comments of contributor \\
ci\_test\_passed   &Whether passed all the CI builds & ci\_first\_build\_status & First build result of CI tool\\
ci\_failed\_perc & Percentage of failed CI builds & ci\_last\_build\_status\ & Last build result of CI tool\\
num\_commits $\dagger$ $\ddagger$ & Number of commits in the pull request & src\_churn $\dagger$ $\ddagger$ & Number of lines changed (added + deleted) by the pull request  \\
files\_added $\dagger$ $\ddagger$ & Number of files added by the pull request & files\_deleted $\dagger$ $\ddagger$ & Number of files deleted by the pull request \\
files\_changed $\dagger$ $\ddagger$ & Number of files touched by the pull request & friday\_effect $\dagger$ $\ddagger$ $\oplus$ & Whether the pull request is submitted on Friday \\
reopen\_or\_not $\dagger$ $\oplus$ & Whether the pull request is reopened or not & commits\_on\_files\_touched $\dagger$ $\ddagger$ & Number of total commits on files touched by the pull request 3 months before the pull request creation time \\
has\_comments $\dagger$ $\ddagger$ $\oplus$ & Whether the pull request has comment & num\_comments $\dagger$ $\ddagger$ & Number of comments in pull request \\
has\_participants $\oplus$ & Whether the pull request has participant & core\_comment $\oplus$ & Whether core member comment in pull request \\
contrib\_comment $\oplus$ & Whether contributor comment in pull request & inte\_comment $\oplus$ & Whether integrator comment in pull request \\
has\_exchange $\oplus$ & Whether contributor and integrator comment together & other\_comment $\dagger$ $\ddagger$ $\oplus$ & Whether others (not contributor or integrator) comment in the pull request \\
num\_comments\_con $\oplus$ & Number of contributors' comments in pull request & at\_tag & Whether @ tag exists in comments or description \\
\bottomrule
\multicolumn{4}{r}{$\dagger$: factors relating to pull request decision; $\ddagger$: factors relating to pull request latency $\oplus$: newly added factors after systematic literature review}\\
%\multirow{2}{*}{\textit{Note:}}  & \multicolumn{3}{r}{$\dagger$: factors relating to pull request decision; $\ddagger$: factors relating to pull request latency} \\ 
%& \multicolumn{3}{r}{$\oplus$: newly added factors after systematic literature review}
\end{tabular}
\end{table*}
\ar{How important is it to identify factors relating to pull request decision and latency when Table 9 captures the same?}

==> tables/decision_after_2013Aug_specific_cases.tex <==
\begin{table*}[!htbp] \centering   \scriptsize
  \caption{The Result for Decision Making Special Case Models} 
  \label{decision_after_2013August_special} 
\begin{tabular}{@{\extracolsep{-20pt}}lD{.}{.}{-3} D{.}{.}{-3} D{.}{.}{-3} D{.}{.}{-3} D{.}{.}{-3} } 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{5}{c}{\textit{Dependent variable: merged\_or\_not=1}} \\ 
\cline{2-6} 
\\[-1.8ex] & \multicolumn{1}{r}{has\_comments=1} & \multicolumn{1}{r}{contrib\_comment=1} & \multicolumn{1}{r}{inte\_comment=1} & \multicolumn{1}{r}{same\_user=0} & \multicolumn{1}{r}{ci\_exists=1}\\ 
\hline \\[-1.8ex] 
 (Intercept) & 15.388^{***} & 11.025^{***} & 9.456^{***} & 32.488^{***} & 26.080^{***} \\ 
  lifetime\_minutes & 0.533^{***}(01) & 0.653^{***}(02) & 0.605^{***}(01) & 0.516^{***}(01) & 0.495^{***}(01) \\
  num\_commits & 1.580^{***}(03) & 1.511^{***}(04) & 1.540^{***}(03) & 1.345^{***}(03) & 1.555^{***}(04) \\
  src\_churn & 1.051^{***}(21) & 1.057^{***}(18) & 1.055^{***}(19) & 1.001^{\,\,\,\,\,\,\,\,\,}(53) & 1.065^{***}(21) \\
  files\_added & 0.913^{***}(15) & 0.896^{***}(12) & 0.889^{***}(11) & 0.958^{**\,\,\,}(29) & 0.904^{***}(16) \\
  files\_deleted & 0.960^{***}(29) & 0.957^{***}(24) & 0.953^{***}(22) & 0.988^{\,\,\,\,\,\,\,\,\,}(43) & 0.961^{***}(25) \\
  files\_changed & 0.943^{***}(18) & 0.961^{***}(26) & 0.961^{***}(24) & 0.913^{***}(15) & 0.970^{***}(28) \\
  friday\_effect & 1.020^{***}(39) & 1.015^{***}(38) & 1.014^{***}(38) & 1.012^{\,\,\,\,\,\,\,\,\,}(44) & 1.015^{***}(40) \\
  reopen\_or\_not & 0.977^{***}(35) & 0.966^{***}(27) & 0.971^{***}(28) & 0.985^{\,\,\,\,\,\,\,\,\,}(40) & 0.977^{***}(34) \\
  commits\_on\_files\_touched & 1.050^{***}(22) & 1.051^{***}(20) & 1.036^{***}(25) & 1.128^{***}(09) & 1.028^{***}(30) \\
  hash\_tag & 1.098^{***}(14) & 1.119^{***}(11) & 1.122^{***}(12) & 1.064^{***}(22) & 1.130^{***}(13) \\
  test\_inclusion & 1.010^{*\,\,\,\,\,\,}(45) & 1.023^{***}(34) & 1.023^{***}(33) & 1.002^{\,\,\,\,\,\,\,\,\,}(50) & 1.020^{***}(37) \\
  description\_length & 1.006^{\,\,\,\,\,\,\,\,\,}(47) & 1.003^{\,\,\,\,\,\,\,\,\,}(44) & 1.011^{***}(40) & 1.018^{\,\,\,\,\,\,\,\,\,}(37) & 1.013^{***}(42) \\
  num\_comments & 0.907^{***}(12) & 1.034^{***}(28) & 1.168^{***}(09) & 0.999^{\,\,\,\,\,\,\,\,\,}(52) & 0.966^{***}(27) \\
  other\_comment & 1.124^{***}(09) & 1.128^{***}(10) & 1.151^{***}(10) & 1.270^{***}(04) & 1.243^{***}(08) \\
  comment\_conflict & 1.016^{***}(41) & 0.999^{\,\,\,\,\,\,\,\,\,}(46) & 1.000^{\,\,\,\,\,\,\,\,\,}(47) & 1.002^{\,\,\,\,\,\,\,\,\,}(51) & 1.009^{***}(44) \\
  test\_churn & 1.109^{***}(10) & 1.091^{***}(15) & 1.089^{***}(16) & 1.104^{***}(11) & 1.119^{***}(14) \\
  prev\_pullreqs & 1.162^{***}(08) & 1.144^{***}(08) & 1.171^{***}(08) & 1.099^{***}(13) & 1.146^{***}(11) \\
  followers & 1.023^{***}(36) & 1.023^{***}(35) & 1.025^{***}(32) & 0.920^{***}(17) & 1.025^{***}(32) \\
  first\_pr & 0.956^{***}(24) & 0.934^{***}(16) & 0.950^{***}(20) & 0.993^{\,\,\,\,\,\,\,\,\,}(47) & 0.956^{***}(23) \\
  account\_creation\_days & 1.059^{***}(19) & 1.047^{***}(21) & 1.049^{***}(21) & 1.161^{***}(06) & 1.090^{***}(17) \\
  core\_member & 1.302^{***}(05) & 1.300^{***}(05) & 1.298^{***}(05) & 1.023^{\,\,\,\,\,\,\,\,\,}(36) & 1.318^{***}(07) \\
  contrib\_gender & 0.974^{***}(32) & 0.976^{***}(32) & 0.973^{***}(30) & 0.932^{***}(20) & 0.980^{***}(35) \\
  contrib\_open & 1.046^{***}(26) & 1.029^{***}(30) & 1.030^{***}(29) & 1.052^{***}(28) & 1.068^{***}(19) \\
  contrib\_cons & 1.046^{***}(25) & 1.056^{***}(19) & 1.047^{***}(23) & 1.043^{**\,\,\,}(30) & 1.028^{***}(31) \\
  contrib\_extra & 0.972^{***}(31) & 0.968^{***}(29) & 0.979^{***}(35) & 0.944^{***}(23) & 0.971^{***}(29) \\
  contrib\_agree & 0.974^{***}(33) & 0.956^{***}(23) & 0.979^{***}(34) & 0.994^{\,\,\,\,\,\,\,\,\,}(48) & 0.980^{***}(36) \\
  contrib\_neur & 1.012^{**\,\,\,}(43) & 1.000^{\,\,\,\,\,\,\,\,\,}(47) & 1.006^{\,\,\,\,\,\,\,\,\,}(42) & 1.068^{***}(21) & 0.998^{\,\,\,\,\,\,\,\,\,}(47)\\
  prior\_review\_num & 1.497^{***}(04) & 1.518^{***}(03) & 1.466^{***}(04) & 1.055^{**\,\,\,}(27) & 1.496^{***}(06) \\
  inte\_open & 1.102^{***}(13) & 1.142^{***}(09) & 1.120^{***}(13) & 1.104^{***}(12) & 0.982^{***}(38) \\
  inte\_cons & 0.997^{\,\,\,\,\,\,\,\,\,}(48) & 0.999^{\,\,\,\,\,\,\,\,\,}(45) & 1.018^{***}(36) & 1.039^{\,\,\,\,\,\,\,\,\,}(31) & 0.993^{\,\,\,\,\,\,\,\,\,}(45)\\
  inte\_extra & 1.011^{*\,\,\,\,\,\,}(44) & 1.004^{\,\,\,\,\,\,\,\,\,}(43) & 1.006^{\,\,\,\,\,\,\,\,\,}(41) & 1.016^{\,\,\,\,\,\,\,\,\,}(39) & 1.059^{***}(22) \\
  inte\_agree & 0.978^{***}(37) & 1.007^{\,\,\,\,\,\,\,\,\,}(41) & 1.001^{\,\,\,\,\,\,\,\,\,}(46) & 0.889^{***}(10) & 1.015^{*\,\,\,\,\,\,}(41) \\
  inte\_neur & 1.035^{***}(30) & 1.046^{***}(22) & 1.031^{***}(27) & 0.995^{\,\,\,\,\,\,\,\,\,}(49) & 0.991^{\,\,\,\,\,\,\,\,\,}(43)\\
  sloc & 1.042^{***}(28) & 1.023^{**\,\,\,}(36) & 1.015^{*\,\,\,\,\,\,}(37) & 0.965^{\,\,\,\,\,\,\,\,\,}(33) & 0.929^{***}(18) \\
  team\_size & 1.056^{***}(20) & 1.041^{***}(25) & 1.057^{***}(18) & 1.015^{\,\,\,\,\,\,\,\,\,}(41) & 1.065^{***}(20) \\
  test\_lines\_per\_kloc & 1.021^{***}(38) & 1.005^{\,\,\,\,\,\,\,\,\,}(42) & 0.999^{\,\,\,\,\,\,\,\,\,}(45) & 0.911^{***}(14) & 1.016^{*\,\,\,\,\,\,}(39) \\
  stars & 0.790^{***}(06) & 0.798^{***}(06) & 0.813^{***}(07) & 0.877^{***}(08) & 0.885^{***}(12) \\
  project\_age & 1.083^{***}(16) & 1.101^{***}(13) & 1.080^{***}(17) & 1.056^{\,\,\,\,\,\,\,\,\,}(25) & 1.212^{***}(09) \\
  open\_issue\_num & 1.019^{\,\,\,\,\,\,\,\,\,}(40) & 0.977^{*\,\,\,\,\,\,}(33) & 1.005^{\,\,\,\,\,\,\,\,\,}(43) & 1.078^{\,\,\,\,\,\,\,\,\,}(18) & 1.025^{\,\,\,\,\,\,\,\,\,}(33)\\
  open\_pr\_num & 0.941^{***}(17) & 0.935^{***}(17) & 0.910^{***}(15) & 1.157^{***}(07) & 0.872^{***}(10) \\
  pr\_succ\_rate & 0.976^{***}(34) & 0.987^{***}(39) & 0.986^{***}(39) & 1.091^{***}(16) & 0.962^{***}(26) \\
  pushed\_delta & 1.044^{***}(27) & 1.027^{***}(31) & 1.032^{***}(26) & 1.058^{***}(24) & 1.043^{***}(24) \\
  integrator\_availability & 1.008^{**\,\,\,}(46) & 0.993^{*\,\,\,\,\,\,}(40) & 0.998^{\,\,\,\,\,\,\,\,\,}(44) & 1.036^{**\,\,\,}(32) & 1.005^{\,\,\,\,\,\,\,\,\,}(46)\\
  
  \hline
  has\_comments &  &  &  & 0.519^{***}(02) & 0.635^{***}(03) \\
  first\_response\_time & 1.014^{***}(42) &  &  &  &  \\ 
  perc\_pos\_emotion & 1.177^{***}(07) &  &  &  &  \\ 
  perc\_neg\_emotion & 0.955^{***}(23) &  &  &  &  \\ 
  
  \hline
  perc\_contrib\_pos\_emo &  & 1.190^{***}(07) &  &  &  \\ 
  perc\_contrib\_neg\_emo &  & 0.982^{***}(37) &  &  &  \\ 
  
  \hline
  perc\_inte\_pos\_emo &  &  & 1.239^{***}(06) &  &  \\ 
  perc\_inte\_neg\_emo &  &  & 1.026^{***}(31) &  &  \\ 
  
  \hline
  same\_user & 0.604^{***}(02) & 0.495^{***}(01) & 0.622^{***}(02) &  & 0.500^{***}(02) \\
  same\_country &  &  &  & 1.015^{\,\,\,\,\,\,\,\,\,}(42) &  \\ 
  same\_affiliation &  &  &  & 1.055^{***}(26) &  \\ 
  contrib\_follow\_integrator &  &  &  & 1.010^{\,\,\,\,\,\,\,\,\,}(45) &  \\ 
  open\_diff &  &  &  & 0.969^{*\,\,\,\,\,\,}(34) &  \\ 
  cons\_diff &  &  &  & 0.984^{\,\,\,\,\,\,\,\,\,}(38) &  \\ 
  extra\_diff &  &  &  & 0.991^{\,\,\,\,\,\,\,\,\,}(46) &  \\ 
  agree\_diff &  &  &  & 0.932^{***}(19) &  \\ 
  neur\_diff &  &  &  & 0.977^{\,\,\,\,\,\,\,\,\,}(35) &  \\ 
  
  \hline
  ci\_exists & 1.108^{***}(11) & 1.100^{***}(14) & 1.116^{***}(14) & 1.252^{***}(05) &  \\ 
  ci\_latency &  &  &  &  & 1.108^{***}(15) \\
  ci\_failed\_perc &  &  &  &  & 0.650^{***}(05) \\
  
 \hline \\[-1.8ex]
Observations & \multicolumn{1}{r}{839,505} & \multicolumn{1}{r}{770,280} & \multicolumn{1}{r}{823,711} & \multicolumn{1}{r}{91,874} & \multicolumn{1}{r}{954,386} \\ 
%Spearman's rank correlation rho & \multicolumn{1}{r}{0.852} & \multicolumn{1}{r}{0.827} & \multicolumn{1}{r}{0.825} & \multicolumn{1}{r}{0.619} & \multicolumn{1}{r}{0.815} \\ 
\hline \\[-1.8ex] 
\hline \\[-1.8ex] 
\multirow{2}{*}{\textit{Note:}} & \multicolumn{5}{r}{odds ratio$^{significance}$(importance ranking)} \\
  & \multicolumn{5}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table*} 

==> tables/decision_after_2013Aug_table.tex <==
\begin{table}[!htbp] \centering
  \scriptsize
  \caption{presents the mixed-effect logistic regression model result for decision making (in non-descending order of percentage of explained variance)} 
  \label{decision_after_2013August_table} 
\begin{tabular}{@{\extracolsep{15pt}}lD{.}{.}{-1} } 
\\[-1.8ex]
\toprule
\\[-3ex] 
 & \multicolumn{1}{r}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & \multicolumn{1}{r}{merged\_or\_not=1} \\ 
\hline \\[-1.8ex] 
 (Intercept) & 21.081^{***} \\ 
  same\_user & 0.524^{***}[31.17] \\
  lifetime\_minutes & 0.608^{***}[21.10] \\
  prior\_review\_num & 1.525^{***}[13.53] \\
  has\_comments & 0.626^{***}[11.97] \\
  core\_member & 1.288^{***}[\,\,\,5.29] \\
  num\_commits & 1.300^{***}[\,\,\,4.49] \\
  other\_comment & 1.212^{***}[\,\,\,3.76] \\
  ci\_exists & 1.159^{***}[\,\,\,1.47] \\
  hash\_tag & 1.115^{***}[\,\,\,1.36] \\
  files\_added & 0.905^{***}[\,\,\,0.74] \\
  prev\_pullreqs & 1.145^{***}[\,\,\,0.73] \\
  commits\_on\_files\_touched & 1.089^{***}[\,\,\,0.59] \\
  open\_pr\_num & 0.815^{***}[\,\,\,0.47] \\
  account\_creation\_days & 1.063^{***}[\,\,\,0.41] \\
  first\_pr & 0.950^{***}[\,\,\,0.36] \\
  test\_churn & 1.071^{***}[\,\,\,0.27] \\
  project\_age & 1.113^{***}[\,\,\,0.26] \\
  files\_changed & 0.921^{***}[\,\,\,0.26] \\
  reopen\_or\_not & 0.967^{***}[\,\,\,0.25] \\
  contrib\_open & 1.060^{***}[\,\,\,0.24] \\
  stars & 0.855^{***}[\,\,\,0.22] \\
  inte\_open & 1.063^{***}[\,\,\,0.21] \\
  description\_length & 1.042^{***}[\,\,\,0.17] \\
  pushed\_delta & 1.038^{***}[\,\,\,0.15] \\
  followers & 1.044^{***}[\,\,\,0.12] \\
  contrib\_cons & 1.034^{***}[\,\,\,0.07] \\
  team\_size & 1.059^{***}[\,\,\,0.06] \\
  contrib\_gender & 0.980^{***}[\,\,\,0.05] \\
  contrib\_gender & 0.980^{***}[\,\,\,0.05] \\
  pr\_succ\_rate & 0.979^{***}[\,\,\,0.03] \\
  files\_deleted & 0.983^{***}[\,\,\,0.03] \\
  num\_comments & 1.023^{***}[\,\,\,0.02] \\
  contrib\_agree & 0.980^{***}[\,\,\,0.02] \\
  inte\_neur & 1.020^{***}[\,\,\,0.02] \\
  contrib\_neur & 1.016^{***}[\,\,\,0.02] \\
  contrib\_extra & 0.985^{***}[\,\,\,0.02] \\
  open\_issue\_num & 1.030^{***}[\,\,\,0.01] \\
  sloc & 1.023^{***}[\,\,\,0.01] \\
  inte\_agree & 1.016^{***}[\,\,\,0.01] \\
  test\_inclusion & 1.015^{***}[\,\,\,0.01] \\
  inte\_extra & 1.013^{***}[\,\,\,0.01] \\
  friday\_effect & 1.010^{***}[\,\,\,0.01] \\
  test\_lines\_per\_kloc & 1.008^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.00]\\
  inte\_cons & 1.008^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.00]\\
  comment\_conflict & 1.006^{***}[\,\,\,0.01] \\
  integrator\_availability & 0.996^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.00]\\
  src\_churn & 1.002^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.00]\\
 \hline \\[-1.8ex] 
Observations\_train & \multicolumn{1}{r}{1,765,730} \\
Observations\_test & \multicolumn{1}{r}{196,192} \\
% Log Likelihood & \multicolumn{1}{r}{-498,621.5} \\ 
% Akaike Inf. Crit. & \multicolumn{1}{r}{997,339} \\ 
% Bayesian Inf. Crit. & \multicolumn{1}{r}{997,933} \\ 
Weighted\_precision\_test & \multicolumn{1}{r}{0.885} \\ 
Weighted\_recall\_test & \multicolumn{1}{r}{0.903} \\
Weighted\_f\_measure\_test & \multicolumn{1}{r}{0.888} \\
AUC\_test & \multicolumn{1}{r}{0.817} \\
AUC\_train & \multicolumn{1}{r}{0.848} \\
\bottomrule
\\[-3ex] 
\multirow{2}{*}{\textit{Note:}} & \multicolumn{1}{r}{odds ratio$^{sig}$(importance ranking)} \\
& \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table}

==> tables/decision_diff_team_size.tex <==
\begin{table}[!htbp] \centering
  \tiny
  \caption{Factors influence on decision making for projects with different team size (in non-descending order of percentage of explained variance for small team)} 
  \label{decision_diff_team_size} 
\begin{tabular}{@{\extracolsep{-53pt}}lD{.}{.}{-3} D{.}{.}{-3} D{.}{.}{-3} } 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{3}{c}{\textit{Dependent variable: merged\_or\_not=1}} \\ 
\cline{2-4} 
\\[-1.8ex] & \multicolumn{1}{r}{Small Team} & \multicolumn{1}{r}{Mid Team} & \multicolumn{1}{r}{Large Team}\\ 
\hline \\[-1.8ex] 
 (Intercept) & 24.853^{***} & 20.673^{***} & 15.928^{***} \\ 
  same\_user & 0.493^{***}[24.47\%] & 0.495^{***}[36.03\%] & 0.545^{***}[32.58\%] \\
  lifetime\_minutes & 0.541^{***}[24.47\%] & 0.611^{***}[20.16\%] & 0.667^{***}[16.55\%] \\
  has\_comments & 0.569^{***}[13.21\%] & 0.640^{***}[10.27\%] & 0.656^{***}[11.93\%] \\
  prior\_review\_num & 1.591^{***}[11.27\%] & 1.414^{***}[\,\,\,8.80\%] & 1.572^{***}[18.89\%] \\
  other\_comment & 1.309^{***}[\,\,\,6.33\%] & 1.234^{***}[\,\,\,4.15\%] & 1.144^{***}[\,\,\,1.92\%] \\
  core\_member & 1.425^{***}[\,\,\,5.90\%] & 1.281^{***}[\,\,\,5.24\%] & 1.187^{***}[\,\,\,3.24\%] \\
  num\_commits & 1.359^{***}[\,\,\,4.64\%] & 1.311^{***}[\,\,\,4.53\%] & 1.265^{***}[\,\,\,4.36\%] \\
  hash\_tag & 1.127^{***}[\,\,\,1.37\%] & 1.108^{***}[\,\,\,1.16\%] & 1.109^{***}[\,\,\,1.38\%] \\
  open\_pr\_num & 0.807^{***}[\,\,\,1.26\%] & 0.830^{***}[\,\,\,0.81\%] & 0.979^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.01\%]\\
  prev\_pullreqs & 1.206^{***}[\,\,\,0.79\%] & 1.213^{***}[\,\,\,1.37\%] & 1.132^{***}[\,\,\,0.84\%] \\
  ci\_exists & 1.132^{***}[\,\,\,0.76\%] & 1.120^{***}[\,\,\,0.79\%] & 1.092^{***}[\,\,\,0.66\%] \\
  watchers & 0.808^{***}[\,\,\,0.69\%] & 0.888^{***}[\,\,\,0.17\%] & 1.046^{**\,\,\,}[\,\,\,0.01\%] \\
  commits\_on\_files\_touched\_close & 1.103^{***}[\,\,\,0.61\%] & 1.116^{***}[\,\,\,0.90\%] & 1.048^{***}[\,\,\,0.20\%] \\
  files\_added & 0.905^{***}[\,\,\,0.52\%] & 0.887^{***}[\,\,\,1.04\%] & 0.903^{***}[\,\,\,0.94\%] \\
  test\_churn & 1.107^{***}[\,\,\,0.45\%] & 1.070^{***}[\,\,\,0.25\%] & 1.042^{***}[\,\,\,0.11\%] \\
  num\_comments & 0.909^{***}[\,\,\,0.37\%] & 1.013^{*\,\,\,\,\,\,}[\,\,\,0.01\%] & 1.130^{***}[\,\,\,0.79\%] \\
  account\_creation\_days & 1.063^{***}[\,\,\,0.33\%] & 1.108^{***}[\,\,\,1.04\%] & 1.022^{***}[\,\,\,0.06\%] \\
  pushed\_delta & 1.057^{***}[\,\,\,0.31\%] & 1.046^{***}[\,\,\,0.25\%] & 1.024^{***}[\,\,\,0.08\%] \\
  team\_size & 1.065^{***}[\,\,\,0.30\%] & 1.000^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.00\%] & 0.958^{***}[\,\,\,0.04\%] \\
  pr\_succ\_rate & 0.939^{***}[\,\,\,0.25\%] & 0.990^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.01\%] & 0.959^{***}[\,\,\,0.10\%] \\
  reopen\_or\_not & 0.967^{***}[\,\,\,0.23\%] & 0.955^{***}[\,\,\,0.48\%] & 0.958^{***}[\,\,\,0.43\%] \\
  first\_pr & 0.952^{***}[\,\,\,0.23\%] & 0.968^{***}[\,\,\,0.15\%] & 0.958^{***}[\,\,\,0.31\%] \\
  files\_changed & 0.928^{***}[\,\,\,0.16\%] & 0.910^{***}[\,\,\,0.33\%] & 0.935^{***}[\,\,\,0.21\%] \\
  contrib\_open & 1.050^{***}[\,\,\,0.12\%] & 1.117^{***}[\,\,\,0.70\%] & 1.049^{***}[\,\,\,0.25\%] \\
  contrib\_cons & 1.051^{***}[\,\,\,0.12\%] & 1.026^{***}[\,\,\,0.04\%] & 1.031^{***}[\,\,\,0.07\%] \\
  inte\_extra & 1.060^{***}[\,\,\,0.11\%] & 1.071^{***}[\,\,\,0.21\%] & 0.955^{***}[\,\,\,0.14\%] \\
  src\_churn & 1.047^{***}[\,\,\,0.10\%] & 1.004^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.00\%] & 0.964^{***}[\,\,\,0.10\%] \\
  contrib\_agree & 0.958^{***}[\,\,\,0.09\%] & 0.993^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.00\%] & 0.982^{***}[\,\,\,0.02\%] \\
  contrib\_gender & 0.969^{***}[\,\,\,0.08\%] & 0.972^{***}[\,\,\,0.09\%] & 0.989^{**\,\,\,}[\,\,\,0.02\%] \\
  description\_length & 1.032^{***}[\,\,\,0.08\%] & 1.026^{***}[\,\,\,0.07\%] & 1.052^{***}[\,\,\,0.29\%] \\
  followers & 1.035^{***}[\,\,\,0.07\%] & 1.006^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.00\%] & 1.075^{***}[\,\,\,0.39\%] \\
  integrator\_availability & 1.025^{***}[\,\,\,0.07\%] & 1.005^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.00\%] & 0.971^{***}[\,\,\,0.14\%] \\
  files\_deleted & 0.973^{***}[\,\,\,0.06\%] & 0.982^{***}[\,\,\,0.04\%] & 0.992^{*\,\,\,\,\,\,}[\,\,\,0.01\%] \\
  inte\_neur & 0.959^{***}[\,\,\,0.05\%] & 0.935^{***}[\,\,\,0.18\%] & 1.095^{***}[\,\,\,0.58\%] \\
  project\_age & 1.044^{***}[\,\,\,0.05\%] & 1.084^{***}[\,\,\,0.15\%] & 0.978^{*\,\,\,\,\,\,}[\,\,\,0.01\%] \\
  comment\_conflict & 1.010^{**\,\,\,}[\,\,\,0.02\%] & 1.001^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.00\%] & 1.010^{***}[\,\,\,0.02\%] \\
  contrib\_extra & 0.980^{***}[\,\,\,0.02\%] & 0.992^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.00\%] & 0.995^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.00\%]\\
  inte\_agree & 1.032^{***}[\,\,\,0.02\%] & 1.009^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.00\%] & 0.977^{***}[\,\,\,0.03\%] \\
  test\_lines\_per\_kloc & 0.979^{**\,\,\,}[\,\,\,0.01\%] & 1.020^{*\,\,\,\,\,\,}[\,\,\,0.01\%] & 0.985^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.01\%]\\
  inte\_open & 0.984^{*\,\,\,\,\,\,}[\,\,\,0.01\%] & 0.924^{***}[\,\,\,0.25\%] & 1.182^{***}[\,\,\,2.12\%] \\
  open\_issue\_num & 1.021^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.01\%] & 1.033^{**\,\,\,}[\,\,\,0.01\%] & 0.963^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.01\%]\\
  friday\_effect & 1.006^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.00\%] & 1.012^{***}[\,\,\,0.02\%] & 1.012^{***}[\,\,\,0.02\%] \\
  test\_inclusion & 0.995^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.00\%] & 1.029^{***}[\,\,\,0.05\%] & 1.015^{**\,\,\,}[\,\,\,0.02\%] \\
  contrib\_neur & 1.004^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.00\%] & 1.074^{***}[\,\,\,0.25\%] & 0.986^{**\,\,\,}[\,\,\,0.02\%] \\
  inte\_cons & 1.006^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.00\%] & 0.999^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.00\%] & 0.987^{**\,\,\,}[\,\,\,0.01\%] \\
  sloc & 0.998^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.00\%] & 0.981^{*\,\,\,\,\,\,}[\,\,\,0.01\%] & 1.073^{***}[\,\,\,0.08\%] \\
 \hline \\[-1.8ex]
Observations & \multicolumn{1}{r}{601,460} & \multicolumn{1}{r}{703,396} & \multicolumn{1}{r}{701,900} \\ 
\hline
\hline \\[-1.8ex] 
\multirow{2}{*}{\textit{Note:}} & \multicolumn{3}{r}{odds ratio$^{significance}$(importance ranking)} \\
  & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 

==> tables/decision_diff_time_period.tex <==
\begin{table}[!htbp] \centering
  \tiny
  \caption{Factors influence on decision making for different time period} 
  \label{decision_diff_time_period} 
\begin{tabular}{@{\extracolsep{-56pt}}lD{.}{.}{-3} D{.}{.}{-3} D{.}{.}{-3} } 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{3}{c}{\textit{Dependent variable: merged\_or\_not=1}} \\ 
\cline{2-4} 
\\[-1.8ex] & \multicolumn{1}{r}{before 2016.6} & \multicolumn{1}{r}{2016.6-2018.6} & \multicolumn{1}{r}{2018.6-2019.6}\\ 
\hline \\[-1.8ex] 
(Intercept) & 6.935^{***} & 16.558^{***} & 7.139^{***} \\ 
  same\_user & 0.571^{***}[31.20\%] & 0.458^{***}[33.20\%] & 0.462^{***}[28.79\%] \\
  lifetime\_minutes & 0.648^{***}[20.26\%] & 0.568^{***}[20.83\%] & 0.622^{***}[12.69\%] \\
  has\_comments & 0.629^{***}[14.94\%] & 0.622^{***}[\,\,\,9.60\%] & 0.549^{***}[13.78\%] \\
  commits\_on\_files\_touched & 1.296^{***}[\,\,\,7.25\%] & 0.991^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.00\%] & 0.994^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.00\%]\\
  prior\_review\_num & 1.297^{***}[\,\,\,6.25\%] & 1.629^{***}[14.12\%] & 1.724^{***}[17.00\%] \\
  core\_member & 1.271^{***}[\,\,\,5.99\%] & 1.343^{***}[\,\,\,4.94\%] & 1.285^{***}[\,\,\,3.14\%] \\
  num\_commits & 1.181^{***}[\,\,\,2.31\%] & 1.320^{***}[\,\,\,4.13\%] & 1.364^{***}[\,\,\,4.84\%] \\
  other\_comment & 1.141^{***}[\,\,\,2.25\%] & 1.224^{***}[\,\,\,3.07\%] & 1.249^{***}[\,\,\,2.84\%] \\
  followers & 1.143^{***}[\,\,\,1.40\%] & 1.057^{***}[\,\,\,0.16\%] & 1.038^{***}[\,\,\,0.07\%] \\
  open\_pr\_num & 0.766^{***}[\,\,\,1.34\%] & 0.723^{***}[\,\,\,0.53\%] & 0.750^{***}[\,\,\,0.28\%] \\
  files\_changed & 0.860^{***}[\,\,\,1.13\%] & 0.948^{***}[\,\,\,0.09\%] & 0.939^{***}[\,\,\,0.13\%] \\
  ci\_exists & 1.085^{***}[\,\,\,0.64\%] & 1.119^{***}[\,\,\,0.44\%] & 1.174^{***}[\,\,\,0.66\%] \\
  first\_pr & 0.949^{***}[\,\,\,0.50\%] & 0.956^{***}[\,\,\,0.20\%] & 0.938^{***}[\,\,\,0.32\%] \\
  contrib\_open & 1.069^{***}[\,\,\,0.46\%] & 1.067^{***}[\,\,\,0.27\%] & 1.020^{**\,\,\,}[\,\,\,0.02\%] \\
  watchers & 0.825^{***}[\,\,\,0.45\%] & 0.723^{***}[\,\,\,0.44\%] & 0.714^{***}[\,\,\,0.50\%] \\
  project\_age & 0.893^{***}[\,\,\,0.40\%] & 1.689^{***}[\,\,\,2.27\%] & 3.798^{***}[\,\,\,4.81\%] \\
  open\_issue\_num & 0.940^{***}[\,\,\,0.04\%] & 1.067^{**\,\,\,}[\,\,\,0.02\%] & 1.046^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.01\%]\\
  team\_size & 0.878^{***}[\,\,\,0.37\%] & 1.088^{***}[\,\,\,0.07\%] & 0.854^{***}[\,\,\,0.16\%] \\
  test\_churn & 1.071^{***}[\,\,\,0.34\%] & 1.100^{***}[\,\,\,0.40\%] & 1.080^{***}[\,\,\,0.23\%] \\
  sloc & 1.127^{***}[\,\,\,0.33\%] & 0.920^{***}[\,\,\,0.07\%] & 0.935^{***}[\,\,\,0.05\%] \\
  num\_comments & 1.076^{***}[\,\,\,0.31\%] & 1.017^{**\,\,\,}[\,\,\,0.01\%] & 1.071^{***}[\,\,\,0.16\%] \\
  prev\_pullreqs & 1.083^{***}[\,\,\,0.29\%] & 1.261^{***}[\,\,\,1.59\%] & 1.240^{***}[\,\,\,1.32\%] \\
  pushed\_delta & 1.044^{***}[\,\,\,0.26\%] & 1.026^{***}[\,\,\,0.05\%] & 1.041^{***}[\,\,\,0.12\%] \\
  test\_lines\_per\_kloc & 1.086^{***}[\,\,\,0.22\%] & 0.949^{***}[\,\,\,0.05\%] & 0.939^{***}[\,\,\,0.06\%] \\
  hash\_tag & 1.040^{***}[\,\,\,0.22\%] & 1.132^{***}[\,\,\,1.44\%] & 1.131^{***}[\,\,\,1.30\%] \\
  pr\_succ\_rate & 0.965^{***}[\,\,\,0.14\%] & 1.004^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.00\%] & 1.106^{***}[\,\,\,0.13\%] \\
  files\_added & 0.966^{***}[\,\,\,0.11\%] & 0.882^{***}[\,\,\,0.95\%] & 0.859^{***}[\,\,\,1.34\%] \\
  inte\_neur & 0.958^{***}[\,\,\,0.11\%] & 0.984^{*\,\,\,\,\,\,}[\,\,\,0.01\%] & 1.125^{***}[\,\,\,0.57\%] \\
  contrib\_agree & 0.975^{***}[\,\,\,0.05\%] & 0.960^{***}[\,\,\,0.08\%] & 1.000^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.00\%]\\
  inte\_open & 0.974^{***}[\,\,\,0.05\%] & 1.030^{***}[\,\,\,0.04\%] & 1.249^{***}[\,\,\,2.21\%] \\
  src\_churn & 0.976^{***}[\,\,\,0.05\%] & 1.006^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.00\%] & 0.995^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.00\%]\\
  files\_deleted & 1.021^{***}[\,\,\,0.05\%] & 0.979^{***}[\,\,\,0.04\%] & 0.971^{***}[\,\,\,0.07\%] \\
  friday\_effect & 1.016^{***}[\,\,\,0.05\%] & 1.009^{*\,\,\,\,\,\,}[\,\,\,0.01\%] & 1.006^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.00\%]\\
  comment\_conflict & 1.015^{***}[\,\,\,0.04\%] & 1.005^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.00\%] & 1.017^{***}[\,\,\,0.04\%] \\
  reopen\_or\_not & 0.989^{***}[\,\,\,0.03\%] & 0.969^{***}[\,\,\,0.18\%] & 0.929^{***}[\,\,\,1.06\%] \\
  contrib\_neur & 1.019^{***}[\,\,\,0.03\%] & 1.024^{***}[\,\,\,0.03\%] & 0.995^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.00\%]\\
  inte\_extra & 1.022^{***}[\,\,\,0.03\%] & 1.043^{***}[\,\,\,0.06\%] & 1.021^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.02\%]\\
  contrib\_cons & 1.013^{**\,\,\,}[\,\,\,0.02\%] & 1.032^{***}[\,\,\,0.05\%] & 1.115^{***}[\,\,\,0.54\%] \\
  contrib\_extra & 0.986^{**\,\,\,}[\,\,\,0.02\%] & 0.966^{***}[\,\,\,0.06\%] & 0.955^{***}[\,\,\,0.11\%] \\
  inte\_agree & 1.019^{**\,\,\,}[\,\,\,0.02\%] & 1.022^{**\,\,\,}[\,\,\,0.01\%] & 0.923^{***}[\,\,\,0.16\%] \\
  description\_length & 0.990^{*\,\,\,\,\,\,}[\,\,\,0.01\%] & 1.060^{***}[\,\,\,0.26\%] & 1.073^{***}[\,\,\,0.36\%] \\
  account\_creation\_days & 0.990^{*\,\,\,\,\,\,}[\,\,\,0.01\%] & 1.018^{***}[\,\,\,0.02\%] & 1.034^{***}[\,\,\,0.06\%] \\
  contrib\_gender & 0.994^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.01\%] & 0.969^{***}[\,\,\,0.10\%] & 1.006^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.00\%]\\
  inte\_cons & 1.013^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.01\%] & 1.027^{***}[\,\,\,0.02\%] & 0.968^{**\,\,\,}[\,\,\,0.03\%] \\
  test\_inclusion & 1.005^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.00\%] & 1.014^{*\,\,\,\,\,\,}[\,\,\,0.01\%] & 1.009^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.00\%]\\
  integrator\_availability & 1.004^{\,\,\,\,\,\,\,\,\,}[\,\,\,0.00\%] & 0.975^{***}[\,\,\,0.06\%] & 0.980^{**\,\,\,}[\,\,\,0.03\%] \\
 \hline \\[-1.8ex] 
Observations & \multicolumn{1}{r}{512,707} & \multicolumn{1}{r}{585,401} & \multicolumn{1}{r}{274,121} \\ 
\hline
\hline \\[-1.8ex] 
\multirow{2}{*}{\textit{Note:}} & \multicolumn{3}{r}{odds ratio$^{significance}$(importance ranking)} \\
  & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table}

==> tables/factor_table.tex <==
\clearpage
\onecolumn
\begin{landscape}
\setlength{\tabcolsep}{0.1em}
\scriptsize
\renewcommand{\arraystretch}{1.6}
\begin{longtable}{l >{\centering}m{0.61cm} >{\centering}m{0.61cm} >{\centering}m{0.61cm} >{\centering}m{0.61cm} >{\centering}m{0.61cm} >{\centering}m{0.61cm} >{\centering}m{0.61cm} >{\centering}m{0.61cm} >{\centering}m{0.61cm} >{\centering}m{0.61cm} >{\centering}m{0.61cm} >{\centering}m{0.61cm} >{\centering}m{0.61cm} >{\centering}m{0.61cm} >{\centering}m{0.61cm} >{\centering}m{0.61cm} >{\centering}m{0.61cm} >{\centering}m{0.61cm} >{\centering}m{0.61cm} >{\centering}m{0.61cm} >{\centering}m{0.61cm} >{\centering}m{0.61cm} >{\centering}m{0.61cm} >{\centering}m{0.61cm} >{\centering}m{0.61cm} >{\centering}m{0.61cm} >{\centering}m{0.61cm} >{\centering}m{0.61cm} >{\centering}m{0.61cm} >{\centering}m{0.61cm} >{\centering}m{0.61cm} c}
\caption{presents relations of factors to pull request decision ($\CIRCLE$) and latency ($\blacktriangle$).
The first column lists the factors and the rest the articles suggesting relations.\\
%Icons are shown in different form, size, and color. 
$\CIRCLE$ shows \emph{quantitative relation} and $\Circle$ shows \emph{qualitative relation}.\\
For quantitative relation, $\CIRCLE$ shows \emph{statistically significant} relation and $\tiny \CIRCLE$ \emph{statistically insignificant}.\\
{\color{blue} $\CIRCLE$} represents a \emph{positive relation} (meaning increase in the chances of pull request acceptance), {\color{red} $\CIRCLE$}  a \emph{negative relation}, and {\color{gray} $\CIRCLE$} an \emph{unclear relation}.
\label{factor_table}}\\
\toprule%
 \centering%
 & {{\bfseries \cite{Gousios_exploratory}}}
 & {{\bfseries \cite{Tsay_influence}}}
 & {{\bfseries \cite{Yu_determinants}}}
 & {{\bfseries \cite{Baysal_investigating}}}
 & {{\bfseries \cite{Iyer_tse}}}
 & {{\bfseries \cite{Iyer_master}}}
 & {{\bfseries \cite{Rastogi_relationshipESEM}}}
 & {{\bfseries \cite{Khadke_predict}}}
 & {{\bfseries \cite{Weigerber_small}}}
 & {{\bfseries \cite{Kononenko_shopify}}}
 & {{\bfseries \cite{Zampetti_ci}}}
 & {{\bfseries \cite{Gousios_integrator}}}
 & {{\bfseries \cite{Soares_acceptance}}}
 & {{\bfseries \cite{Soares_rejection}}}
 & {{\bfseries \cite{Golzadeh_discussion}}}
 & {{\bfseries \cite{Padhye_external}}}
 & {{\bfseries \cite{Legay_impact}}}
 & {{\bfseries \cite{Jiang_reopen}}}
 & {{\bfseries \cite{Rahman_insight}}}
 & {{\bfseries \cite{Baysal_firefox}}}
 & {{\bfseries \cite{Pinto_who}}}
 & {{\bfseries \cite{Bosu_reputation}}}
 & {{\bfseries \cite{Lee_onetime}}}
 & {{\bfseries \cite{Hechtl_coreness}}}
 & {{\bfseries \cite{Kovalenko_newcomer}}}
 & {{\bfseries \cite{Terrell_gender}}}
 & {{\bfseries \cite{Yu_wait}}}
 & {{\bfseries \cite{Bernardo_ci}}}
 & {{\bfseries \cite{Hilton_ci}}}
 & {{\bfseries \cite{Zhao_ci}}}
 & {{\bfseries \cite{Imtiaz_gender}}}
 & {{\bfseries \cite{Sadowski_google}}} \\
\endhead

\rowcolor[gray]{0.925}
lifetime\_minutes & & & & & & & & & & & \textcolor{red}{\normalsize $\Circle$} & & \textcolor{red}{\normalsize $\Circle$} & & & & \textcolor{red}{\normalsize $\Circle$} & & & & & & & & & & & & & & & \\

num\_commits & \textcolor{gray}{\normalsize $\Circle$}\textcolor{gray}{\normalsize $\triangle$} & & \textcolor{blue}{\normalsize $\CIRCLE$}\textcolor{blue}{\normalsize $\blacktriangle$} & & & & & \textcolor{red}{\normalsize $\Circle$} & & \textcolor{gray}{\normalsize $\Circle$} & \textcolor{gray}{\normalsize $\Circle$} & & \textcolor{red}{\normalsize $\Circle$} & \textcolor{red}{\normalsize $\Circle$} & & & & & & & & & & & & & \textcolor{red}{\normalsize $\blacktriangle$} & & & & & \\

\rowcolor[gray]{0.925}
src\_churn & \textcolor{gray}{\normalsize $\Circle$}\textcolor{gray}{\normalsize $\triangle$} & \textcolor{red}{\normalsize $\CIRCLE$} & & \textcolor{gray}{\normalsize $\Circle$} & \textcolor{red}{\normalsize $\CIRCLE$} & \textcolor{red}{\normalsize $\CIRCLE$} & \textcolor{red}{\normalsize $\CIRCLE$} & \textcolor{red}{\normalsize $\Circle$} & \textcolor{red}{\normalsize $\Circle$} & \textcolor{red}{\normalsize $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & & & \\

test\_churn & \textcolor{gray}{\normalsize $\Circle$}\textcolor{gray}{\normalsize $\triangle$} & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & \\

\rowcolor[gray]{0.925}
files\_added & & & & & & & & & & & & & \textcolor{red}{\normalsize $\Circle$} & & & & & & & & & & & & & & & & & & & \\

files\_deleted & & & & & & & & & & & & & \textcolor{blue}{\normalsize $\Circle$} & & & & & & & & & & & & & & & & & & & \\

\rowcolor[gray]{0.925}
files\_changed & \textcolor{gray}{\normalsize $\Circle$}\textcolor{gray}{\normalsize $\triangle$} & \textcolor{red}{\normalsize $\CIRCLE$} & & & \textcolor{gray}{\normalsize $\Circle$} & \textcolor{gray}{\normalsize $\Circle$} & \textcolor{blue}{\tiny $\CIRCLE$} & \textcolor{blue}{\normalsize $\Circle$} & & \textcolor{gray}{\normalsize $\Circle$} & \textcolor{gray}{\normalsize $\Circle$} & & \textcolor{gray}{\normalsize $\Circle$} & \textcolor{red}{\normalsize $\Circle$} & & & & & & & & & & & & & & & & & & \\

num\_comments & \textcolor{gray}{\normalsize $\Circle$} & \textcolor{red}{\normalsize $\CIRCLE$} & \textcolor{red}{\normalsize $\CIRCLE$} & & \textcolor{red}{\normalsize $\CIRCLE$} & \textcolor{red}{\normalsize $\CIRCLE$} & \textcolor{red}{\normalsize $\CIRCLE$} & & & \textcolor{gray}{\normalsize $\Circle$} & \textcolor{gray}{\normalsize $\Circle$} & & & & & & & & & & & & & & & & & & & & & \\

\rowcolor[gray]{0.925}
num\_participants & \textcolor{gray}{\normalsize $\Circle$}\textcolor{gray}{\normalsize $\triangle$} & & & & & & & & & \textcolor{red}{\normalsize $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & & & \\

sloc & \textcolor{gray}{\normalsize $\Circle$}\textcolor{gray}{\normalsize $\triangle$} & & & & & & \textcolor{red}{\normalsize $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & & & & & & \\

\rowcolor[gray]{0.925}
team\_size & \textcolor{gray}{\normalsize $\Circle$}\textcolor{gray}{\normalsize $\triangle$} & \textcolor{red}{\normalsize $\CIRCLE$} & \textcolor{blue}{\tiny $\CIRCLE$}\textcolor{blue}{\normalsize $\blacktriangle$} & & \textcolor{red}{\tiny $\CIRCLE$} & \textcolor{red}{\tiny $\CIRCLE$} & & \textcolor{blue}{\normalsize $\Circle$} & & & & & & & & & & & \textcolor{gray}{\normalsize $\Circle$} & & & & & & & & \textcolor{blue}{\normalsize $\blacktriangle$} & & & & & \\

perc\_external\_contribs & \textcolor{gray}{\normalsize $\Circle$}\textcolor{gray}{\normalsize $\triangle$} & & & & & & \textcolor{red}{\normalsize $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & & & & & & \\

\rowcolor[gray]{0.925}
commits\_on\_files\_touched & \textcolor{gray}{\normalsize $\Circle$}\textcolor{gray}{\normalsize $\triangle$} & & \textcolor{blue}{\normalsize $\CIRCLE$}\textcolor{red}{\normalsize $\blacktriangle$} & & & & & & & & & & & & & & & & & & & & & & & & \textcolor{red}{\normalsize $\blacktriangle$} & & & & & \\

test\_lines\_per\_kloc & \textcolor{gray}{\normalsize $\Circle$}\textcolor{gray}{\normalsize $\triangle$} & & & & & & \textcolor{blue}{\normalsize $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & & & & & & \\

\rowcolor[gray]{0.925}
test\_cases\_per\_kloc & \textcolor{gray}{\normalsize $\Circle$}\textcolor{gray}{\normalsize $\triangle$} & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & \\

asserts\_per\_kloc & \textcolor{gray}{\normalsize $\Circle$}\textcolor{gray}{\normalsize $\triangle$} & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & \\

\rowcolor[gray]{0.925}
stars & & \textcolor{red}{\normalsize $\CIRCLE$} & & & \textcolor{red}{\normalsize $\CIRCLE$} & \textcolor{red}{\normalsize $\CIRCLE$} & \textcolor{red}{\normalsize $\CIRCLE$} & \textcolor{red}{\normalsize $\Circle$} & & & & & & & & & & & & & & & & & & & & & & & & \\

prev\_pullreqs & \textcolor{gray}{\normalsize $\Circle$}\textcolor{gray}{\normalsize $\triangle$} & & & \textcolor{blue}{\normalsize $\CIRCLE$} & & & \textcolor{blue}{\normalsize $\CIRCLE$} & & & \textcolor{blue}{\normalsize $\CIRCLE$} & & & & & & & \textcolor{blue}{\normalsize $\Circle$} & & & & & & & & & & & & & & & \\

\rowcolor[gray]{0.925}
requester\_succ\_rate & \textcolor{gray}{\normalsize $\Circle$}\textcolor{gray}{\normalsize $\triangle$} & & & & & & \textcolor{blue}{\normalsize $\CIRCLE$} & \textcolor{blue}{\normalsize $\Circle$} & & & \textcolor{gray}{\normalsize $\Circle$} & & & & & & & & & & & & & & & & \textcolor{blue}{\normalsize $\blacktriangle$} & & & & & \\

followers & & \textcolor{blue}{\normalsize $\CIRCLE$}\textcolor{blue}{\normalsize $\blacktriangle$} & \textcolor{blue}{\normalsize $\CIRCLE$} & & \textcolor{gray}{\tiny $\CIRCLE$} & \textcolor{gray}{\tiny $\CIRCLE$} & \textcolor{blue}{\normalsize $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & \textcolor{blue}{\normalsize $\blacktriangle$} & & & & & \\

\rowcolor[gray]{0.925}
churn\_addition & & & \textcolor{red}{\normalsize $\CIRCLE$}\textcolor{red}{\normalsize $\blacktriangle$} & & & & & & & & & & & & & & & & & & & & & & & & \textcolor{red}{\normalsize $\blacktriangle$} & & & & & \\


churn\_deletion & & & \textcolor{blue}{\normalsize $\CIRCLE$}\textcolor{blue}{\tiny $\blacktriangle$} & & & & & & & & \textcolor{gray}{\normalsize $\Circle$} & & & & & & & & & & & & & & & & \textcolor{blue}{\tiny $\blacktriangle$} & & & & & \\

\rowcolor[gray]{0.925}
perc\_neg\_emotion & & & & & & \textcolor{red}{\normalsize $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & & & & & & & \\


perc\_pos\_emotion & & & & & & \textcolor{blue}{\normalsize $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & & & & & & & \\

\rowcolor[gray]{0.925}
part\_num\_code & & & & & & & & & & \textcolor{blue}{\normalsize $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & & & \\


comment\_conflict & \textcolor{gray}{\normalsize $\Circle$}\textcolor{gray}{\normalsize $\triangle$} & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & \\

\rowcolor[gray]{0.925}
hash\_tag & \textcolor{gray}{\normalsize $\Circle$}\textcolor{gray}{\normalsize $\triangle$} & & \textcolor{blue}{\tiny $\CIRCLE$}\textcolor{red}{\normalsize $\blacktriangle$} & & & & & & & & & & & & & & & & & & & & & & & & \textcolor{red}{\normalsize $\blacktriangle$} & & & & & \\


at\_tag & & & \textcolor{blue}{\tiny $\CIRCLE$}\textcolor{blue}{\tiny $\blacktriangle$} & & & & & & & & & & & & & & & & & & & & & & & & \textcolor{blue}{\tiny $\blacktriangle$} & & & & & \\

\rowcolor[gray]{0.925}
test\_inclusion & & \textcolor{blue}{\normalsize $\CIRCLE$} & \textcolor{blue}{\normalsize $\CIRCLE$}\textcolor{red}{\normalsize $\blacktriangle$} & & \textcolor{blue}{\normalsize $\CIRCLE$} & \textcolor{blue}{\normalsize $\CIRCLE$} & \textcolor{blue}{\normalsize $\CIRCLE$} & & & & \textcolor{gray}{\normalsize $\Circle$} & \textcolor{blue}{\normalsize $\Circle$} & & & & & & & & & & & & & & & \textcolor{red}{\tiny $\blacktriangle$} & & & & & \\


description\_length & & & \textcolor{red}{\normalsize $\CIRCLE$}\textcolor{red}{\normalsize $\blacktriangle$} & & & & & & & & & & & & & & & & & & & & & & & & \textcolor{red}{\normalsize $\blacktriangle$} & & & & & \\

\rowcolor[gray]{0.925}
bug\_fix & & & & & & & & & & & \textcolor{blue}{\normalsize $\Circle$} & & & & & \textcolor{blue}{\normalsize $\Circle$} & & & & & & & & & & & & & & & & \\


ci\_exists & & & & & & & & & & & & & & & & & & & & & & & & & & & & \textcolor{red}{\normalsize $\triangle$} & \textcolor{red}{\normalsize $\CIRCLE$}\textcolor{blue}{\normalsize $\blacktriangle$} & \textcolor{red}{\tiny $\blacktriangle$} & & \\

\rowcolor[gray]{0.925}
ci\_latency & & & \textcolor{blue}{\normalsize $\CIRCLE$}\textcolor{red}{\normalsize $\blacktriangle$} & & & & & & & & & & & & & & & & & & & & & & & & \textcolor{red}{\normalsize $\blacktriangle$} & & & & & \\


ci\_build\_num & & & & & & & & & & & \textcolor{gray}{\normalsize $\Circle$} & & & & & & & & & & & & & & & & & & & & & \\

\rowcolor[gray]{0.925}
ci\_test\_passed & & & \textcolor{blue}{\normalsize $\CIRCLE$}\textcolor{blue}{\normalsize $\blacktriangle$} & & & & & & & & & \textcolor{blue}{\normalsize $\Circle$} & & & & & & & & & & & & & & & \textcolor{red}{\normalsize $\blacktriangle$} & & & & & \\


ci\_failed\_perc & & & & & & & & & & & \textcolor{gray}{\normalsize $\Circle$} & & & & & & & & & & & & & & & & & & & & & \\

\rowcolor[gray]{0.925}
ci\_first\_build\_status & & & & & & & & & & & \textcolor{blue}{\normalsize $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & & \\


ci\_last\_build\_status & & & & & & & & & & & \textcolor{blue}{\normalsize $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & & \\

\rowcolor[gray]{0.925}
language & & & & & & & & & & & & & \textcolor{gray}{\normalsize $\Circle$} & & & & & & \textcolor{gray}{\normalsize $\Circle$} & & & & & & & & & & & & & \\


fork\_num & & & & & & & & \textcolor{red}{\normalsize $\Circle$} & & & & & & & & & & & \textcolor{red}{\normalsize $\Circle$} & & & & & & & & & & & & & \\

\rowcolor[gray]{0.925}
project\_age & & \textcolor{red}{\normalsize $\CIRCLE$}\textcolor{red}{\normalsize $\blacktriangle$} & \textcolor{blue}{\normalsize $\CIRCLE$} & & \textcolor{red}{\normalsize $\CIRCLE$} & \textcolor{red}{\normalsize $\CIRCLE$} & \textcolor{red}{\normalsize $\CIRCLE$} & & & & & & & & & & & & \textcolor{red}{\normalsize $\Circle$} & & & & & & & & \textcolor{blue}{\normalsize $\blacktriangle$} & & & & & \\


open\_issue\_num & & & & & & & & \textcolor{blue}{\normalsize $\Circle$} & & & & & & & & & & & & & & & & & & & & & & & & \\

\rowcolor[gray]{0.925}
pr\_succ\_rate & & & & & & & & \textcolor{blue}{\normalsize $\Circle$} & & & & & & & & & & & & & & & & & & & & & & & & \\


open\_pr\_num & & & \textcolor{red}{\normalsize $\CIRCLE$}\textcolor{red}{\normalsize $\blacktriangle$} & \textcolor{blue}{\normalsize $\Circle$} & & & & & & & & & & & & & & & & & & & & & & & \textcolor{red}{\normalsize $\blacktriangle$} & & & & & \\

\rowcolor[gray]{0.925}
first\_response\_time & & & \textcolor{red}{\normalsize $\CIRCLE$}\textcolor{red}{\normalsize $\blacktriangle$} & & & & & & & & & & & & & & & & & & & & & & & & \textcolor{red}{\normalsize $\blacktriangle$} & & & & & \\


pushed\_delta & & & & & & & & \textcolor{red}{\normalsize $\Circle$} & & & & & & & & & & & & & & & & & & & & & & & & \\

\rowcolor[gray]{0.925}
first\_pr & & & & & & & & & & & & & \textcolor{red}{\normalsize $\Circle$} & \textcolor{red}{\normalsize $\Circle$} & & & & & & & & & \textcolor{red}{\normalsize $\CIRCLE$} & & \textcolor{red}{\normalsize $\Circle$} & & & & & & & \\

account\_creation\_days & & & & & & & \textcolor{red}{\normalsize $\CIRCLE$} & & & & & & & & & & & & \textcolor{gray}{\normalsize $\Circle$} & & & & & & & & & & & & & \\

\rowcolor[gray]{0.925}
core\_member & & \textcolor{blue}{\normalsize $\CIRCLE$} & \textcolor{blue}{\normalsize $\CIRCLE$}\textcolor{blue}{\normalsize $\blacktriangle$} & & \textcolor{blue}{\normalsize $\CIRCLE$} & \textcolor{blue}{\normalsize $\CIRCLE$} & \textcolor{blue}{\tiny $\CIRCLE$} & & & & \textcolor{blue}{\normalsize $\Circle$} & & \textcolor{blue}{\normalsize $\Circle$} & & & & & & & \textcolor{blue}{\normalsize $\Circle$} & \textcolor{blue}{\normalsize $\Circle$} & \textcolor{blue}{\normalsize $\Circle$} & \textcolor{blue}{\normalsize $\CIRCLE$} & \textcolor{gray}{\normalsize $\Circle$} & & & \textcolor{blue}{\normalsize $\blacktriangle$} & & & & & \\

contrib\_gender & & & & & & & & & & & & & & & & & & & & & & & & & & \textcolor{blue}{\normalsize $\Circle$} & & & & & \textcolor{blue}{\normalsize $\triangle$} & \\

\rowcolor[gray]{0.925}
contrib\_country & & & & & & & \textcolor{gray}{\normalsize $\Circle$} & & & & & & & & & & & & & & & & & & & & & & & & & \\

contrib\_affiliation & & & & \textcolor{gray}{\normalsize $\Circle$} & & & & & & \textcolor{gray}{\normalsize $\CIRCLE$}\textcolor{gray}{\normalsize $\blacktriangle$} & & & & & & & & & & & & & & & & & & & & & & \\

\rowcolor[gray]{0.925}
contrib\_open & & & & & \textcolor{blue}{\normalsize $\CIRCLE$} & \textcolor{blue}{\normalsize $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & & & & & & & \\

contrib\_cons & & & & & \textcolor{blue}{\normalsize $\CIRCLE$} & \textcolor{blue}{\normalsize $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & & & & & & & \\

\rowcolor[gray]{0.925}
contrib\_extra & & & & & \textcolor{red}{\normalsize $\CIRCLE$} & \textcolor{red}{\normalsize $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & & & & & & & \\

contrib\_agree & & & & & \textcolor{blue}{\tiny $\CIRCLE$} & \textcolor{blue}{\tiny $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & & & & & & & \\

\rowcolor[gray]{0.925}
contrib\_neur & & & & & \textcolor{red}{\tiny $\CIRCLE$} & \textcolor{red}{\tiny $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & & & & & & & \\

perc\_contrib\_neg\_emo & & & & & & \textcolor{red}{\normalsize $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & & & & & & & \\

\rowcolor[gray]{0.925}
perc\_contrib\_pos\_emo & & & & & & \textcolor{blue}{\normalsize $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & & & & & & & \\

contrib\_first\_emo & & & & & & \textcolor{blue}{\normalsize $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & & & & & & & \\

\rowcolor[gray]{0.925}
prior\_review\_num & & & & \textcolor{gray}{\tiny $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & & & & & & & & & \\

inte\_affiliation & & & & \textcolor{gray}{\normalsize $\Circle$} & & & & & & & & & & & & & & & & & & & & & & & & & & & & \textcolor{gray}{\normalsize $\triangle$} \\

\rowcolor[gray]{0.925}
inte\_open & & & & & \textcolor{blue}{\normalsize $\CIRCLE$} & \textcolor{blue}{\normalsize $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & & & & & & & \\

inte\_cons & & & & & \textcolor{blue}{\normalsize $\CIRCLE$} & \textcolor{blue}{\normalsize $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & & & & & & & \\

\rowcolor[gray]{0.925}
inte\_extra & & & & & \textcolor{blue}{\normalsize $\CIRCLE$} & \textcolor{blue}{\normalsize $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & & & & & & & \\

inte\_agree & & & & & \textcolor{blue}{\tiny $\CIRCLE$} & \textcolor{blue}{\tiny $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & & & & & & & \\

\rowcolor[gray]{0.925}
inte\_neur & & & & & \textcolor{blue}{\normalsize $\CIRCLE$} & \textcolor{blue}{\normalsize $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & & & & & & & \\

perc\_inte\_neg\_emo & & & & & & \textcolor{red}{\normalsize $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & & & & & & & \\

\rowcolor[gray]{0.925}
perc\_inte\_pos\_emo & & & & & & \textcolor{blue}{\normalsize $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & & & & & & & \\

inte\_first\_emo & & & & & & \textcolor{blue}{\normalsize $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & & & & & & & \\

\rowcolor[gray]{0.925}
contrib\_follow\_integrator & & \textcolor{blue}{\normalsize $\CIRCLE$} & & & \textcolor{blue}{\normalsize $\CIRCLE$} & \textcolor{blue}{\normalsize $\CIRCLE$} & \textcolor{blue}{\normalsize $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & & & & & & \\

prior\_interaction & & \textcolor{blue}{\normalsize $\CIRCLE$} & & & \textcolor{blue}{\normalsize $\CIRCLE$} & \textcolor{blue}{\normalsize $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & & & & & & & \\

\rowcolor[gray]{0.925}
social\_strength & & & \textcolor{blue}{\normalsize $\CIRCLE$}\textcolor{blue}{\tiny $\blacktriangle$} & & & & & & & & & & & & & & & & & & & & & & & & \textcolor{blue}{\normalsize $\blacktriangle$} & & & & & \\

same\_country & & & & & & & \textcolor{blue}{\normalsize $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & & & & & & \\

\rowcolor[gray]{0.925}
same\_affiliation & & & & \textcolor{blue}{\normalsize $\Circle$} & & & & & & & & & & & & & & & & & & & & & & & & & & & & \\

open\_diff & & & & & \textcolor{blue}{\tiny $\CIRCLE$} & \textcolor{blue}{\tiny $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & & & & & & & \\

\rowcolor[gray]{0.925}
cons\_diff & & & & & \textcolor{blue}{\normalsize $\CIRCLE$} & \textcolor{blue}{\normalsize $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & & & & & & & \\

extra\_diff & & & & & \textcolor{blue}{\normalsize $\CIRCLE$} & \textcolor{blue}{\normalsize $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & & & & & & & \\

\rowcolor[gray]{0.925}
agree\_diff & & & & & \textcolor{blue}{\normalsize $\CIRCLE$} & \textcolor{blue}{\normalsize $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & & & & & & & \\

neur\_diff & & & & & \textcolor{blue}{\normalsize $\CIRCLE$} & \textcolor{blue}{\normalsize $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & & & & & & & \\

\rowcolor[gray]{0.925}
has\_comments & & & & & & & & & & & & & & \textcolor{red}{\normalsize $\Circle$} & \textcolor{red}{\normalsize $\Circle$} & & & & & & & & & & & & & & & & & \\

has\_participants & & & & & & & & & & & & & & & \textcolor{red}{\normalsize $\Circle$} & & & & & & & & & & & & & & & & & \\

\rowcolor[gray]{0.925}
has\_exchange & & & & & & & & & & & & & & & \textcolor{red}{\normalsize $\Circle$} & & & & & & & & & & & & & & & & & \\

contrib\_comment & & & & & & & & & & & & & & & \textcolor{red}{\normalsize $\Circle$} & & & & & & & & & & & & & & & & & \\

\rowcolor[gray]{0.925}
inte\_comment & & & & & & & & & & & & & & & \textcolor{blue}{\normalsize $\Circle$} & & & & & & & & & & & & & & & & & \\

core\_comment & & & & & & & & & & & & & & & \textcolor{red}{\normalsize $\Circle$} & & & & & & & & & & & & & & & & & \\

\rowcolor[gray]{0.925}
other\_comment & & & & & & & & & & & & & & & \textcolor{red}{\normalsize $\Circle$} & & & & & & & & & & & & & & & & & \\

num\_comments\_con & & & & & & & & & & \textcolor{gray}{\tiny $\CIRCLE$} & & & & & & & & & & & & & & & & & & & & & & \\

\rowcolor[gray]{0.925}
num\_code\_comments & & & & & & & & & & \textcolor{gray}{\normalsize $\Circle$} & \textcolor{gray}{\normalsize $\Circle$} & & & & & & & & & & & & & & & & & & & & & \\

num\_code\_comments\_con & & & & & & & & & & \textcolor{gray}{\normalsize $\Circle$} & & & & & & & & & & & & & & & & & & & & & & \\

\rowcolor[gray]{0.925}
integrator\_availability & & & \textcolor{red}{\normalsize $\CIRCLE$}\textcolor{red}{\normalsize $\blacktriangle$} & & & & & & & & & & & & & & & & & & & & & & & & \textcolor{red}{\normalsize $\blacktriangle$} & & & & & \\

friday\_effect & & & \textcolor{blue}{\tiny $\CIRCLE$}\textcolor{red}{\normalsize $\blacktriangle$} & & & & & & & & & & & & & & & & & & & & & & & & \textcolor{red}{\normalsize $\blacktriangle$} & & & & & \\

\rowcolor[gray]{0.925}
contrib\_rate\_author & & & & & & & & & & & \textcolor{gray}{\normalsize $\Circle$} & & & & & & & & & & & & & & & & & & & & & \\

reopen\_or\_not & & & & & & & & & & & & & & & & & & \textcolor{red}{\normalsize $\Circle$}\textcolor{red}{\normalsize $\triangle$} & & & & & & & & & & & & & & \\

\bottomrule

\end{longtable}
\end{landscape}
\normalsize
\twocolumn
\clearpage

==> tables/latency_after_2013Aug_specific_cases.tex <==
\begin{table*}[!htbp] \centering 
\scriptsize
  \caption{The result of latency after August 2013 with special cases} 
  \label{latency_after_2013August_special} 
\begin{tabular}{@{\extracolsep{-70pt}}lD{.}{.}{-3} D{.}{.}{-3} D{.}{.}{-3} D{.}{.}{-3} D{.}{.}{-3} } 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{5}{c}{\textit{Dependent variable: log(lifetime\_minutes+1)}} \\ 
\cline{2-6} 
 & \multicolumn{1}{r}{has\_comments=1} & \multicolumn{1}{r}{contrib\_comment=1} & \multicolumn{1}{r}{inte\_comment=1} & \multicolumn{1}{r}{same\_user=0} &  \multicolumn{1}{r}{ci\_exists=1} \\  
\hline \\[-1.8ex] 
 Constant & 1764.367^{***} & 3271.691^{***} & 2808.486^{***} & 1220.927^{***} & 1228.018^{***} \\ 
  num\_commits & 1.117^{***}(\,\,\,0.31\%)(11) & 1.201^{***}(\,\,\,2.60\%)(06) & 1.199^{***}(\,\,\,2.26\%)(09) & 1.237^{***}(\,\,\,4.04\%)(06) & 1.253^{***}(\,\,\,4.04\%)(08) \\
  src\_churn & 1.135^{***}(\,\,\,0.37\%)(09) & 1.233^{***}(\,\,\,3.12\%)(05) & 1.263^{***}(\,\,\,3.41\%)(05) & 1.276^{***}(\,\,\,4.80\%)(03) & 1.249^{***}(\,\,\,3.66\%)(09) \\
  files\_added & 0.987^{***}(\,\,\,0.00\%)(37) & 1.000^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.00\%)(41) & 1.002^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.00\%)(40) & 0.966^{***}(\,\,\,0.11\%)(32) & 1.033^{***}(\,\,\,0.09\%)(24) \\
  files\_deleted & 0.963^{***}(\,\,\,0.05\%)(20) & 0.937^{***}(\,\,\,0.48\%)(17) & 0.930^{***}(\,\,\,0.53\%)(19) & 0.937^{***}(\,\,\,0.56\%)(17) & 0.942^{***}(\,\,\,0.43\%)(16) \\
  files\_changed & 1.013^{***}(\,\,\,0.00\%)(38) & 1.029^{***}(\,\,\,0.03\%)(32) & 1.032^{***}(\,\,\,0.04\%)(30) & 1.096^{***}(\,\,\,0.42\%)(20) & 0.994^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.00\%)(36) \\
  friday\_effect & 1.060^{***}(\,\,\,0.19\%)(15) & 1.089^{***}(\,\,\,1.24\%)(10) & 1.088^{***}(\,\,\,1.11\%)(11) & 1.103^{***}(\,\,\,1.84\%)(09) & 1.079^{***}(\,\,\,1.03\%)(13) \\
  commits\_on\_files\_touched & 0.914^{***}(\,\,\,0.23\%)(13) & 0.895^{***}(\,\,\,1.08\%)(12) & 0.896^{***}(\,\,\,0.95\%)(14) & 0.869^{***}(\,\,\,2.18\%)(08) & 0.884^{***}(\,\,\,1.38\%)(11) \\
  hash\_tag & 1.154^{***}(\,\,\,0.91\%)(04) & 1.191^{***}(\,\,\,4.01\%)(02) & 1.192^{***}(\,\,\,3.69\%)(04) & 1.148^{***}(\,\,\,2.84\%)(07) & 1.192^{***}(\,\,\,4.25\%)(07) \\
  test\_inclusion & 1.011^{***}(\,\,\,0.00\%)(39) & 1.013^{***}(\,\,\,0.01\%)(36) & 1.009^{**\,\,\,}(\,\,\,0.00\%)(41) & 1.018^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.02\%)(42) & 1.003^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.00\%)(37) \\
  description\_length & 1.128^{***}(\,\,\,0.57\%)(06) & 1.193^{***}(\,\,\,3.84\%)(03) & 1.212^{***}(\,\,\,4.14\%)(02) & 1.206^{***}(\,\,\,4.29\%)(05) & 1.223^{***}(\,\,\,4.90\%)(06) \\
  num\_comments & 2.247^{***}(21.31\%)(02) & 2.324^{***}(66.84\%)(01) & 2.371^{***}(64.15\%)(01) & 2.723^{***}(54.04\%)(01) & 2.299^{***}(35.53\%)(01) \\
  other\_comment & 1.338^{***}(\,\,\,3.14\%)(03) & 1.097^{***}(\,\,\,0.96\%)(14) & 1.088^{***}(\,\,\,0.72\%)(15) & 1.014^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.02\%)(43) & 1.010^{***}(\,\,\,0.01\%)(32) \\
  comment\_conflict & 1.075^{***}(\,\,\,0.28\%)(12) & 1.121^{***}(\,\,\,2.12\%)(07) & 1.118^{***}(\,\,\,1.81\%)(10) & 1.060^{***}(\,\,\,0.61\%)(16) & 1.086^{***}(\,\,\,1.15\%)(12) \\
  test\_churn & 0.991^{***}(\,\,\,0.00\%)(40) & 1.020^{***}(\,\,\,0.02\%)(33) & 1.024^{***}(\,\,\,0.03\%)(31) & 1.080^{***}(\,\,\,0.38\%)(22) & 1.034^{***}(\,\,\,0.07\%)(25) \\
    prev\_pullreqs & 0.855^{***}(\,\,\,0.35\%)(10) & 0.850^{***}(\,\,\,1.14\%)(11) & 0.847^{***}(\,\,\,1.07\%)(12) & 0.938^{***}(\,\,\,0.24\%)(26) & 0.931^{***}(\,\,\,0.22\%)(19) \\
  followers & 0.972^{***}(\,\,\,0.02\%)(25) & 0.934^{***}(\,\,\,0.35\%)(20) & 0.938^{***}(\,\,\,0.28\%)(22) & 1.000^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.00\%)(48) & 0.945^{***}(\,\,\,0.23\%)(18) \\
  first\_pr & 1.039^{***}(\,\,\,0.05\%)(21) & 1.009^{***}(\,\,\,0.01\%)(37) & 1.012^{***}(\,\,\,0.01\%)(36) & 1.042^{***}(\,\,\,0.20\%)(28) & 1.036^{***}(\,\,\,0.13\%)(23) \\
  account\_creation\_days & 0.984^{***}(\,\,\,0.01\%)(31) & 0.987^{***}(\,\,\,0.02\%)(34) & 0.988^{***}(\,\,\,0.01\%)(37) & 0.976^{**\,\,\,}(\,\,\,0.05\%)(37) & 0.986^{***}(\,\,\,0.02\%)(31) \\
  core\_member & 0.916^{***}(\,\,\,0.19\%)(16) & 0.918^{***}(\,\,\,0.56\%)(16) & 0.912^{***}(\,\,\,0.56\%)(18) & 0.941^{***}(\,\,\,0.33\%)(23) & 0.895^{***}(\,\,\,0.94\%)(14) \\
  contrib\_gender & 0.996^{**\,\,\,}(\,\,\,0.00\%)(42) & 0.999^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.00\%)(43) & 0.999^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.00\%)(42) & 1.008^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.01\%)(45) & 1.007^{***}(\,\,\,0.01\%)(33) \\
  contrib\_open & 0.972^{***}(\,\,\,0.02\%)(26) & 0.972^{***}(\,\,\,0.07\%)(27) & 0.967^{***}(\,\,\,0.08\%)(27) & 0.969^{***}(\,\,\,0.08\%)(33) & 0.995^{*\,\,\,\,\,\,}(\,\,\,0.00\%)(38) \\
  contrib\_cons & 0.964^{***}(\,\,\,0.03\%)(23) & 0.967^{***}(\,\,\,0.09\%)(25) & 0.964^{***}(\,\,\,0.09\%)(25) & 0.944^{***}(\,\,\,0.28\%)(24) & 0.970^{***}(\,\,\,0.07\%)(26) \\
  contrib\_extra & 1.030^{***}(\,\,\,0.02\%)(27) & 1.036^{***}(\,\,\,0.09\%)(26) & 1.035^{***}(\,\,\,0.09\%)(26) & 1.054^{***}(\,\,\,0.22\%)(27) & 0.999^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.00\%)(39) \\
  contrib\_agree & 0.981^{***}(\,\,\,0.01\%)(32) & 0.975^{***}(\,\,\,0.04\%)(30) & 0.969^{***}(\,\,\,0.07\%)(28) & 0.975^{**\,\,\,}(\,\,\,0.05\%)(38) & 0.990^{***}(\,\,\,0.01\%)(34) \\
  contrib\_neur & 0.980^{***}(\,\,\,0.01\%)(33) & 1.003^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.00\%)(44) & 0.992^{**\,\,\,}(\,\,\,0.00\%)(43) & 0.994^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.00\%)(49) & 0.994^{*\,\,\,\,\,\,}(\,\,\,0.00\%)(40) \\
  prior\_review\_num & 1.052^{***}(\,\,\,0.06\%)(19) & 1.082^{***}(\,\,\,0.43\%)(19) & 1.103^{***}(\,\,\,0.63\%)(17) & 1.113^{***}(\,\,\,0.80\%)(14) & 1.009^{***}(\,\,\,0.01\%)(35) \\
  inte\_open & 1.068^{***}(\,\,\,0.08\%)(18) & 1.139^{***}(\,\,\,0.91\%)(15) & 1.088^{***}(\,\,\,0.37\%)(21) & 1.199^{***}(\,\,\,1.43\%)(11) & 1.068^{***}(\,\,\,0.21\%)(20) \\
  inte\_cons & 1.037^{***}(\,\,\,0.02\%)(28) & 1.057^{***}(\,\,\,0.17\%)(22) & 1.072^{***}(\,\,\,0.23\%)(23) & 1.088^{***}(\,\,\,0.39\%)(21) & 1.036^{***}(\,\,\,0.06\%)(28) \\
  inte\_extra & 0.986^{***}(\,\,\,0.00\%)(43) & 0.973^{***}(\,\,\,0.04\%)(31) & 0.976^{***}(\,\,\,0.03\%)(32) & 0.929^{***}(\,\,\,0.27\%)(25) & 0.999^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.00\%)(41) \\
  inte\_agree & 0.972^{***}(\,\,\,0.01\%)(34) & 0.979^{***}(\,\,\,0.02\%)(35) & 0.995^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.00\%)(44) & 0.938^{***}(\,\,\,0.17\%)(29) & 0.994^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.00\%)(42) \\
  inte\_neur & 1.052^{***}(\,\,\,0.05\%)(22) & 1.063^{***}(\,\,\,0.24\%)(21) & 1.092^{***}(\,\,\,0.43\%)(20) & 1.113^{***}(\,\,\,0.63\%)(15) & 1.057^{***}(\,\,\,0.15\%)(22) \\
  sloc & 1.004^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.00\%)(44) & 0.977^{***}(\,\,\,0.01\%)(38) & 0.979^{***}(\,\,\,0.01\%)(38) & 0.965^{*\,\,\,\,\,\,}(\,\,\,0.03\%)(41) & 0.991^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.00\%)(43) \\
  team\_size & 0.947^{***}(\,\,\,0.02\%)(29) & 0.849^{***}(\,\,\,0.46\%)(18) & 0.816^{***}(\,\,\,0.67\%)(16) & 0.853^{***}(\,\,\,0.52\%)(18) & 0.920^{***}(\,\,\,0.17\%)(21) \\
  test\_lines\_per\_kloc & 0.975^{***}(\,\,\,0.01\%)(35) & 0.958^{***}(\,\,\,0.06\%)(28) & 0.952^{***}(\,\,\,0.07\%)(29) & 0.961^{**\,\,\,}(\,\,\,0.06\%)(36) & 0.951^{***}(\,\,\,0.07\%)(27) \\
  watchers & 0.968^{***}(\,\,\,0.00\%)(45) & 0.976^{**\,\,\,}(\,\,\,0.01\%)(39) & 0.969^{***}(\,\,\,0.01\%)(39) & 0.893^{***}(\,\,\,0.15\%)(31) & 0.933^{***}(\,\,\,0.04\%)(29) \\
  project\_age & 1.058^{***}(\,\,\,0.03\%)(24) & 1.051^{***}(\,\,\,0.06\%)(29) & 1.032^{***}(\,\,\,0.02\%)(33) & 1.029^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.02\%)(44) & 0.988^{**\,\,\,}(\,\,\,0.00\%)(44) \\
  open\_issue\_num & 1.004^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.00\%)(46) & 0.996^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.00\%)(45) & 1.002^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.00\%)(45) & 0.995^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.00\%)(51) & 0.983^{*\,\,\,\,\,\,}(\,\,\,0.00\%)(45) \\
  open\_pr\_num & 1.359^{***}(\,\,\,0.41\%)(07) & 1.529^{***}(\,\,\,2.03\%)(09) & 1.592^{***}(\,\,\,2.33\%)(08) & 1.841^{***}(\,\,\,4.58\%)(04) & 1.627^{***}(\,\,\,3.27\%)(10) \\
  pr\_succ\_rate & 1.020^{***}(\,\,\,0.01\%)(36) & 1.015^{***}(\,\,\,0.01\%)(40) & 1.019^{***}(\,\,\,0.02\%)(34) & 1.022^{**\,\,\,}(\,\,\,0.04\%)(39) & 1.027^{***}(\,\,\,0.04\%)(30) \\
  pushed\_delta & 1.063^{***}(\,\,\,0.15\%)(17) & 1.095^{***}(\,\,\,1.00\%)(13) & 1.104^{***}(\,\,\,1.06\%)(13) & 1.109^{***}(\,\,\,1.45\%)(10) & 1.087^{***}(\,\,\,0.94\%)(15) \\
  integrator\_availability & 1.071^{***}(\,\,\,0.21\%)(14) & 1.177^{***}(\,\,\,3.59\%)(04) & 1.201^{***}(\,\,\,4.08\%)(03) & 1.289^{***}(\,\,\,9.29\%)(02) & 1.215^{***}(\,\,\,5.50\%)(05) \\
  
  \hline
  has\_comments &  &  &  & 1.006^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.00\%)(47) & 1.066^{***}(\,\,\,0.27\%)(17) \\
  first\_response\_time & 3.753^{***}(69.65\%)(01) &  &  &  &  \\ 
  perc\_pos\_emotion & 0.871^{***}(\,\,\,0.82\%)(05) &  &  &  &  \\ 
  perc\_neg\_emotion & 0.998^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.00\%)(41) &  &  &  &  \\ 
  
  \hline
  perc\_contrib\_pos\_emo &  & 0.997^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.00\%)(42) &  &  &  \\ 
  perc\_contrib\_neg\_emo &  & 0.977^{***}(\,\,\,0.09\%)(24) &  &  &  \\ 
  
  \hline
  perc\_inte\_pos\_emo &  &  & 0.861^{***}(\,\,\,2.49\%)(06) &  &  \\ 
  perc\_inte\_neg\_emo &  &  & 0.991^{***}(\,\,\,0.01\%)(35) &  &  \\ 
  
  
  \hline
  same\_user & 0.893^{***}(\,\,\,0.38\%)(08) & 0.861^{***}(\,\,\,2.03\%)(08) & 0.837^{***}(\,\,\,2.34\%)(07) &  & 0.773^{***}(\,\,\,6.22\%)(03) \\
  same\_country &  &  &  & 0.939^{***}(\,\,\,0.43\%)(19) &  \\ 
  same\_affiliation &  &  &  & 0.906^{***}(\,\,\,0.96\%)(12) &  \\ 
  contrib\_follow\_integrator &  &  &  & 1.022^{**\,\,\,}(\,\,\,0.06\%)(35) &  \\ 
  open\_diff &  &  &  & 0.970^{***}(\,\,\,0.07\%)(34) &  \\ 
  cons\_diff &  &  &  & 0.998^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.00\%)(50) &  \\ 
  extra\_diff &  &  &  & 0.990^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.01\%)(46) &  \\ 
  agree\_diff &  &  &  & 1.041^{***}(\,\,\,0.16\%)(30) &  \\ 
  neur\_diff &  &  &  & 1.021^{*\,\,\,\,\,\,}(\,\,\,0.03\%)(40) &  \\ 
  
  \hline
  ci\_exists & 1.015^{***}(\,\,\,0.01\%)(30) & 1.041^{***}(\,\,\,0.12\%)(23) & 1.036^{***}(\,\,\,0.09\%)(24) & 1.105^{***}(\,\,\,0.84\%)(13) &  \\ 
  ci\_latency &  &  &  &  & 1.515^{***}(18.76\%)(02) \\
  ci\_failed\_perc &  &  &  &  & 1.230^{***}(\,\,\,6.12\%)(04) \\
 \hline \\[-1.8ex]
Observations & \multicolumn{1}{r}{823,138} & \multicolumn{1}{r}{750,378} & \multicolumn{1}{r}{804,511} & \multicolumn{1}{r}{90,560} & \multicolumn{1}{r}{939,433} \\ 
%Spearman's rank correlation rho & \multicolumn{1}{r}{0.781} & \multicolumn{1}{r}{0.840} & \multicolumn{1}{r}{0.850} & \multicolumn{1}{r}{0.728} & \multicolumn{1}{r}{0.891} \\ 
\hline 
\hline \\[-1.8ex] 
\multirow{2}{*}{\textit{Note:}} & \multicolumn{5}{r}{exp(coef)$^{sig}$(Sum of Square proportion)(rank)} \\
& \multicolumn{5}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table*}

==> tables/latency_after_2013Aug_table.tex <==
\begin{table}[!htbp] \centering 
\scriptsize
  \caption{Mixed-effect linear regression model results for latency} 
  \label{latency_after_2013August_table} 
\begin{tabular}{@{\extracolsep{-20pt}}lD{.}{.}{-3} } 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & \multicolumn{1}{c}{log(lifetime\_minutes+1)} \\ 
\hline \\[-1.8ex] 
 (Intercept) & 694.376^{***} \\ 
  num\_commits & 1.285^{***}(\,\,\,4.13\%)(06)\\
  src\_churn & 1.299^{***}(\,\,\,4.23\%)(05)\\
  files\_added & 0.977^{***}(\,\,\,0.04\%)(28)\\
  files\_deleted & 0.915^{***}(\,\,\,0.77\%)(15)\\
  files\_changed & 1.014^{***}(\,\,\,0.01\%)(33)\\
  friday\_effect & 1.070^{***}(\,\,\,0.69\%)(16)\\
  commits\_on\_files\_touched & 0.892^{***}(\,\,\,1.02\%)(13)\\
  hash\_tag & 1.164^{***}(\,\,\,2.64\%)(08)\\
  test\_inclusion & 1.002^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.00\%)(42)\\
  description\_length & 1.410^{***}(11.34\%)(03)\\
  ci\_exists & 1.164^{***}(\,\,\,1.30\%)(11)\\
  has\_comments & 1.242^{***}(\,\,\,2.48\%)(09)\\
  comment\_conflict & 1.077^{***}(\,\,\,0.78\%)(14)\\
  num\_comments & 2.650^{***}(39.24\%)(01)\\
  other\_comment & 1.037^{***}(\,\,\,0.11\%)(23)\\
  test\_churn & 1.058^{***}(\,\,\,0.17\%)(20)\\
  followers & 0.953^{***}(\,\,\,0.13\%)(21)\\
  first\_pr & 1.025^{***}(\,\,\,0.06\%)(25)\\
  account\_creation\_days & 0.989^{***}(\,\,\,0.01\%)(34)\\
  core\_member & 0.870^{***}(\,\,\,1.33\%)(10)\\
  contrib\_gender & 0.990^{***}(\,\,\,0.01\%)(35)\\
  contrib\_open & 0.979^{***}(\,\,\,0.03\%)(29)\\
  contrib\_cons & 0.958^{***}(\,\,\,0.11\%)(24)\\
  contrib\_extra & 0.986^{***}(\,\,\,0.01\%)(36)\\
  contrib\_agree & 0.989^{***}(\,\,\,0.01\%)(37)\\
  contrib\_neur & 0.985^{***}(\,\,\,0.01\%)(38)\\
  prev\_pullreqs & 0.962^{***}(\,\,\,0.06\%)(26)\\
  prior\_review\_num & 1.010^{***}(\,\,\,0.01\%)(39)\\
  inte\_open & 1.128^{***}(\,\,\,0.59\%)(17)\\
  inte\_cons & 1.058^{***}(\,\,\,0.13\%)(22)\\
  inte\_extra & 0.974^{***}(\,\,\,0.03\%)(30)\\
  inte\_agree & 0.980^{***}(\,\,\,0.01\%)(40)\\
  inte\_neur & 1.067^{***}(\,\,\,0.18\%)(19)\\
  same\_user & 0.629^{***}(17.40\%)(02)\\
  sloc & 0.954^{***}(\,\,\,0.03\%)(31)\\
  team\_size & 0.874^{***}(\,\,\,0.30\%)(18)\\
  test\_lines\_per\_kloc & 0.987^{***}(\,\,\,0.00\%)(43)\\
  stars & 0.958^{***}(\,\,\,0.01\%)(41)\\
  project\_age & 1.053^{***}(\,\,\,0.05\%)(27)\\
  open\_issue\_num & 0.979^{***}(\,\,\,0.00\%)(44)\\
  open\_pr\_num & 1.847^{***}(\,\,\,3.98\%)(07)\\
  pr\_succ\_rate & 1.023^{***}(\,\,\,0.02\%)(32)\\
  pushed\_delta & 1.110^{***}(\,\,\,1.17\%)(12)\\
  integrator\_availability & 1.235^{***}(\,\,\,5.37\%)(04)\\
 \hline \\[-1.8ex] 
Observations\_train & \multicolumn{1}{r}{1,740,905} \\ 
Observations\_test & \multicolumn{1}{r}{193,434} \\ 
% Log Likelihood & \multicolumn{1}{r}{-3,935,964} \\ 
% AIC & \multicolumn{1}{r}{7,872,021} \\ 
% BIC & \multicolumn{1}{r}{7,872,602} \\ 
% R2m & \multicolumn{1}{r}{0.364} \\ 
% R2c & \multicolumn{1}{r}{0.472} \\ 
MAE\_test & \multicolumn{1}{r}{1.8794} \\
MSE\_test & \multicolumn{1}{r}{5.5255} \\
\hline 
\hline \\[-1.8ex] 
\multirow{2}{*}{\textit{Note:}} & \multicolumn{1}{r}{exp(coef)$^{sig}$(Sum of Square proportion)(rank)} \\
& \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 

==> tables/latency_after_2013Aug_table_5models.tex <==
\begin{table*}[!htbp] \centering 
  \caption{Mixed-effect linear regression model results for latency} 
  \label{latency_after_2013August_table} 
\begin{tabular}{@{\extracolsep{-45pt}}lD{.}{.}{-3} D{.}{.}{-3} D{.}{.}{-3} D{.}{.}{-3} D{.}{.}{-3} } 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{5}{c}{\textit{Dependent variable: lifetime\_minutes}} \\ 
\cline{2-6} 
\\[-1.8ex] & \multicolumn{1}{c}{Model1} & \multicolumn{1}{c}{Model2} & \multicolumn{1}{c}{Model3} & \multicolumn{1}{c}{Model4} & \multicolumn{1}{c}{Model5}\\ 
\hline \\[-1.8ex] 
 (Intercept) & 0.057^{***} & 0.027^{***} & 0.031^{***} & 0.033^{***} & -0.019^{***} \\ 
  num\_commits & 0.046(12.7\%)^{***} & 0.045(10.3\%)^{***} & 0.045(9.4\%)^{***} & 0.045(9.8\%)^{***} & 0.046(8.5\%)^{***} \\ 
  src\_churn & 0.002(0\%)^{**} & 0.002(0\%)^{**} & 0.002(0\%)^{**} & 0.002(0\%)^{**} & 0.001(0\%)^{*} \\ 
  files\_added & 0.011(0.5\%)^{***} & 0.009(0.3\%)^{***} & 0.010(0.3\%)^{***} & 0.010(0.3\%)^{***} & 0.008(0.2\%)^{***} \\ 
  files\_deleted & -0.0002(0\%) & -0.0003(0\%) & -0.0001(0\%) & -0.0001(0\%) & -0.001(0\%)\\
  files\_changed & -0.011(0.3\%)^{***} & -0.010(0.2\%)^{***} & -0.010(0.2\%)^{***} & -0.010(0.2\%)^{***} & -0.008(0.1\%)^{***} \\ 
  friday\_effect & 0.003(0.1\%)^{***} & 0.003(0.1\%)^{***} & 0.003(0.1\%)^{***} & 0.003(0.1\%)^{***} & 0.004(0.1\%)^{***} \\ 
  commits\_on\_files\_touched & -0.008(0.4\%)^{***} & -0.006(0.2\%)^{***} & -0.005(0.1\%)^{***} & -0.005(0.1\%)^{***} & -0.010(0.4\%)^{***} \\ 
  hash\_tag & 0.035(8.3\%)^{***} & 0.037(7.9\%)^{***} & 0.036(7.1\%)^{***} & 0.036(7.2\%)^{***} & 0.038(7\%)^{***} \\ 
  test\_inclusion & 0.019(2.4\%)^{***} & 0.023(3\%)^{***} & 0.023(2.8\%)^{***} & 0.023(2.9\%)^{***} & 0.023(2.5\%)^{***} \\ 
  description\_length & 0.033(6.4\%)^{***} & 0.030(4.6\%)^{***} & 0.029(4.1\%)^{***} & 0.029(4.1\%)^{***} & 0.034(4.7\%)^{***} \\ 
  ci\_exists & -0.019(1.3\%)^{***} & -0.007(0.2\%)^{***} & -0.008(0.2\%)^{***} & -0.008(0.2\%)^{***} & 0.010(0.2\%)^{***} \\ 
  has\_comments & 0.101(67.6\%)^{***} & 0.088(42.9\%)^{***} & 0.089(40.1\%)^{***} & 0.088(39.8\%)^{***} & 0.086(32.5\%)^{***} \\ 
  followers &  & -0.005(0.1\%)^{***} & -0.005(0.1\%)^{***} & -0.004(0.1\%)^{***} & -0.003(0\%)^{***} \\ 
  first\_pr &  & 0.042(9.6\%)^{***} & 0.042(8.9\%)^{***} & 0.041(8.9\%)^{***} & 0.039(6.6\%)^{***} \\ 
  account\_creation\_days &  & -0.028(3.7\%)^{***} & -0.030(3.8\%)^{***} & -0.029(3.6\%)^{***} & -0.005(0.1\%)^{***} \\ 
  core\_member &  & -0.056(14.5\%)^{***} & -0.056(13.4\%)^{***} & -0.052(11.1\%)^{***} & -0.050(8.8\%)^{***} \\ 
  contrib\_gender &  & 0.006(0.2\%)^{***} & 0.006(0.2\%)^{***} & 0.006(0.2\%)^{***} & 0.001(0\%)^{*} \\ 
  contrib\_open &  & -0.007(0.1\%)^{***} & -0.016(0.7\%)^{***} & -0.017(0.8\%)^{***} & -0.018(0.7\%)^{***} \\ 
  contrib\_cons &  & -0.021(1.5\%)^{***} & -0.027(2\%)^{***} & -0.026(1.9\%)^{***} & -0.020(0.9\%)^{***} \\ 
  contrib\_extra &  & 0.012(0.5\%)^{***} & 0.018(0.9\%)^{***} & 0.019(1.1\%)^{***} & 0.016(0.6\%)^{***} \\ 
  contrib\_agree &  & -0.004(0.1\%)^{***} & -0.005(0.1\%)^{***} & -0.005(0.1\%)^{***} & -0.004(0\%)^{***} \\ 
  contrib\_neur &  & -0.006(0.1\%)^{***} & -0.015(0.5\%)^{***} & -0.015(0.6\%)^{***} & -0.011(0.2\%)^{***} \\ 
  prior\_review\_num &  &  & 0.012(0.5\%)^{***} & 0.010(0.3\%)^{***} & 0.033(3\%)^{***} \\ 
  inte\_open &  &  & 0.034(2.2\%)^{***} & 0.037(2.6\%)^{***} & 0.041(2.8\%)^{***} \\ 
  inte\_cons &  &  & 0.017(0.6\%)^{***} & 0.016(0.5\%)^{***} & 0.019(0.6\%)^{***} \\ 
  inte\_extra &  &  & -0.017(0.5\%)^{***} & -0.019(0.7\%)^{***} & -0.023(0.9\%)^{***} \\ 
  inte\_agree &  &  & 0.001(0\%) & 0.001(0\%) & -0.001(0\%)\\
  inte\_neur &  &  & 0.026(1.3\%)^{***} & 0.028(1.4\%)^{***} & 0.030(1.4\%)^{***} \\ 
  same\_user &  &  &  & -0.018(1.4\%)^{***} & -0.017(1.1\%)^{***} \\ 
  sloc &  &  &  &  & -0.001(0\%)\\
  team\_size &  &  &  &  & 0.021(0.2\%)^{***} \\ 
  test\_lines\_per\_kloc &  &  &  &  & 0.0004(0\%)\\
  stars &  &  &  &  & -0.047(1.4\%)^{***} \\ 
  project\_age &  &  &  &  & -0.084(7.4\%)^{***} \\ 
  open\_issue\_num &  &  &  &  & 0.041(1.1\%)^{***} \\ 
  open\_pr\_num &  &  &  &  & -0.100(3.5\%)^{***} \\ 
  pr\_succ\_rate &  &  &  &  & -0.023(1\%)^{***} \\ 
  pushed\_delta &  &  &  &  & 0.013(0.8\%)^{***} \\ 
  integrator\_availability &  &  &  &  & 0.012(0.7\%)^{***} \\ 
 \hline \\[-1.8ex] 
Observations\_training & \multicolumn{1}{c}{1,740,905} & \multicolumn{1}{c}{1,740,905} & \multicolumn{1}{c}{1,740,905} & \multicolumn{1}{c}{1,740,905} & \multicolumn{1}{c}{1,740,905} \\ 
Observations\_testing & \multicolumn{1}{c}{193,434} & \multicolumn{1}{c}{193,434} & \multicolumn{1}{c}{193,434} & \multicolumn{1}{c}{193,434} & \multicolumn{1}{c}{193,434} \\ 
Deviance & \multicolumn{1}{c}{4,719,539} & \multicolumn{1}{c}{4,705,837} & \multicolumn{1}{c}{4,704,730} & \multicolumn{1}{c}{4,704,357} & \multicolumn{1}{c}{4,696,202} \\
Log Likelihood & \multicolumn{1}{c}{-2,359,769} & \multicolumn{1}{c}{-2,352,919} & \multicolumn{1}{c}{-2,352,365} & \multicolumn{1}{c}{-2,352,179} & \multicolumn{1}{c}{-2,348,101} \\ 
AIC & \multicolumn{1}{c}{4,719,569} & \multicolumn{1}{c}{4,705,887} & \multicolumn{1}{c}{4,704,792} & \multicolumn{1}{c}{4,704,421} & \multicolumn{1}{c}{4,696,286} \\ 
BIC & \multicolumn{1}{c}{4,719,754} & \multicolumn{1}{c}{4,706,196} & \multicolumn{1}{c}{4,705,176} & \multicolumn{1}{c}{4,704,817} & \multicolumn{1}{c}{4,696,806} \\ 
MAE\_test & \multicolumn{1}{c}{0.3137} & \multicolumn{1}{c}{0.3061} & \multicolumn{1}{c}{0.3072} & \multicolumn{1}{c}{0.3074} & \multicolumn{1}{c}{0.3086} \\
MSE\_test & \multicolumn{1}{c}{1.3822} & \multicolumn{1}{c}{1.3708} & \multicolumn{1}{c}{1.3681} & \multicolumn{1}{c}{1.3676} & \multicolumn{1}{c}{1.3703} \\
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{5}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table*}

==> tables/latency_diff_team_size.tex <==
\begin{table*}[!htbp] \centering 
\scriptsize
  \caption{Factors influence on latency for projects with different team size} 
  \label{latency_diff_team_size} 
\begin{tabular}{@{\extracolsep{-10pt}}lD{.}{.}{-3} D{.}{.}{-3} D{.}{.}{-3} } 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{3}{c}{\textit{Dependent variable: lifetime\_minutes}} \\ 
\cline{2-4} 
 & \multicolumn{1}{r}{Small Team} & \multicolumn{1}{r}{Mid Team} & \multicolumn{1}{r}{Large Team} \\ 
\hline \\[-1.8ex] 
 (Intercept) & 802.334^{***} & 791.330^{***} & 705.206^{***} \\ 
  \textbf{num\_commits} & 1.523^{***}(\,\,\,3.04\%)(07) & 1.408^{***}(\,\,\,8.58\%)(04) & 1.243^{***}(13.32\%)(04) \\
  src\_churn & 1.263^{***}(\,\,\,4.31\%)(05) & 1.286^{***}(\,\,\,3.91\%)(09) & 1.302^{***}(\,\,\,3.36\%)(09) \\
  files\_added & 0.987^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.05\%)(28) & 0.981^{***}(\,\,\,0.03\%)(31) & 0.974^{***}(\,\,\,0.01\%)(37) \\
  files\_deleted & 0.924^{***}(\,\,\,0.73\%)(16) & 0.917^{***}(\,\,\,0.94\%)(13) & 0.915^{***}(\,\,\,0.82\%)(13) \\
  files\_changed & 1.025^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.00\%)(41) & 1.055^{***}(\,\,\,0.11\%)(19) & 1.007^{*\,\,\,\,\,\,}(\,\,\,0.02\%)(35) \\
  friday\_effect & 1.065^{***}(\,\,\,0.65\%)(17) & 1.074^{***}(\,\,\,0.84\%)(14) & 1.069^{***}(\,\,\,0.66\%)(14) \\
  commits\_on\_files\_touched & 0.948^{***}(\,\,\,1.19\%)(11) & 0.905^{***}(\,\,\,0.75\%)(15) & 0.885^{***}(\,\,\,0.19\%)(19) \\
  hash\_tag & 1.235^{***}(\,\,\,2.35\%)(08) & 1.213^{***}(\,\,\,3.96\%)(08) & 1.152^{***}(\,\,\,4.42\%)(07) \\
  test\_inclusion & 0.976^{**\,\,\,}(\,\,\,0.00\%)(42) & 0.992^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.00\%)(41) & 1.007^{**\,\,\,}(\,\,\,0.04\%)(32) \\
  description\_length & 1.508^{***}(10.83\%)(03) & 1.454^{***}(13.69\%)(03) & 1.395^{***}(15.83\%)(02) \\
  ci\_exists & 1.134^{***}(\,\,\,1.04\%)(12) & 1.166^{***}(\,\,\,1.44\%)(11) & 1.143^{***}(\,\,\,0.89\%)(12) \\
  \textbf{has\_comments} & 1.515^{***}(\,\,\,2.04\%)(09) & 1.347^{***}(\,\,\,4.47\%)(06) & 1.217^{***}(\,\,\,7.72\%)(05) \\
  comment\_conflict & 1.071^{***}(\,\,\,0.86\%)(14) & 1.075^{***}(\,\,\,0.43\%)(16) & 1.077^{***}(\,\,\,0.33\%)(16) \\
  \textbf{num\_comments} & 2.045^{***}(43.02\%)(01) & 2.325^{***}(23.96\%)(01) & 2.721^{***}(14.96\%)(03) \\
  other\_comment & 0.995^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.16\%)(21) & 0.999^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.00\%)(42) & 1.043^{***}(\,\,\,0.00\%)(38) \\
  test\_churn & 1.088^{***}(\,\,\,0.17\%)(20) & 1.056^{***}(\,\,\,0.16\%)(18) & 1.059^{***}(\,\,\,0.39\%)(15) \\
  followers & 0.996^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.14\%)(22) & 0.963^{***}(\,\,\,0.07\%)(26) & 0.953^{***}(\,\,\,0.00\%)(39) \\
  first\_pr & 0.967^{***}(\,\,\,0.06\%)(27) & 1.016^{**\,\,\,}(\,\,\,0.02\%)(34) & 1.026^{***}(\,\,\,0.05\%)(29) \\
  account\_creation\_days & 1.020^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.01\%)(34) & 0.979^{***}(\,\,\,0.03\%)(32) & 0.991^{***}(\,\,\,0.02\%)(36) \\
  core\_member & 0.819^{***}(\,\,\,1.30\%)(10) & 0.862^{***}(\,\,\,1.33\%)(12) & 0.873^{***}(\,\,\,1.97\%)(10) \\
  contrib\_gender & 0.976^{**\,\,\,}(\,\,\,0.01\%)(35) & 1.015^{***}(\,\,\,0.02\%)(35) & 0.990^{***}(\,\,\,0.05\%)(30) \\
  contrib\_open & 1.004^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.03\%)(30) & 0.990^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.00\%)(43) & 0.977^{***}(\,\,\,0.00\%)(40) \\
  contrib\_cons & 0.938^{***}(\,\,\,0.11\%)(23) & 0.956^{***}(\,\,\,0.10\%)(21) & 0.959^{***}(\,\,\,0.16\%)(22) \\
  contrib\_extra & 0.921^{***}(\,\,\,0.00\%)(43) & 0.969^{***}(\,\,\,0.05\%)(28) & 0.992^{***}(\,\,\,0.29\%)(17) \\
  contrib\_agree & 1.073^{***}(\,\,\,0.02\%)(31) & 0.985^{*\,\,\,\,\,\,}(\,\,\,0.01\%)(36) & 0.982^{***}(\,\,\,0.17\%)(21) \\
  contrib\_neur & 1.009^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.01\%)(36) & 0.989^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.01\%)(37) & 0.984^{***}(\,\,\,0.00\%)(41) \\
  prev\_pullreqs & 0.956^{**\,\,\,}(\,\,\,0.09\%)(25) & 0.960^{***}(\,\,\,0.04\%)(29) & 0.952^{***}(\,\,\,0.04\%)(33) \\
  prior\_review\_num & 1.048^{**\,\,\,}(\,\,\,0.01\%)(37) & 0.983^{*\,\,\,\,\,\,}(\,\,\,0.01\%)(38) & 1.011^{***}(\,\,\,0.05\%)(31) \\
  inte\_open & 1.060^{***}(\,\,\,0.77\%)(15) & 1.053^{***}(\,\,\,0.08\%)(24) & 1.140^{***}(\,\,\,0.08\%)(26) \\
  inte\_cons & 1.062^{***}(\,\,\,0.10\%)(24) & 1.053^{***}(\,\,\,0.11\%)(20) & 1.051^{***}(\,\,\,0.12\%)(24) \\
  inte\_extra & 0.994^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.02\%)(32) & 0.969^{***}(\,\,\,0.04\%)(30) & 0.977^{***}(\,\,\,0.00\%)(42) \\
  inte\_agree & 0.920^{***}(\,\,\,0.01\%)(38) & 0.957^{***}(\,\,\,0.06\%)(27) & 0.984^{***}(\,\,\,0.18\%)(20) \\
  inte\_neur & 0.990^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.24\%)(19) & 1.048^{***}(\,\,\,0.09\%)(23) & 1.075^{***}(\,\,\,0.00\%)(43) \\
  \textbf{same\_user} & 0.598^{***}(16.06\%)(02) & 0.608^{***}(21.30\%)(02) & 0.638^{***}(21.97\%)(01) \\
  sloc & 1.012^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.07\%)(26) & 0.980^{*\,\,\,\,\,\,}(\,\,\,0.01\%)(39) & 0.931^{***}(\,\,\,0.00\%)(44) \\
  team\_size & 1.093^{***}(\,\,\,0.37\%)(18) & 0.916^{***}(\,\,\,0.10\%)(22) & 0.866^{***}(\,\,\,0.07\%)(27) \\
  test\_lines\_per\_kloc & 1.060^{***}(\,\,\,0.01\%)(39) & 1.019^{*\,\,\,\,\,\,}(\,\,\,0.01\%)(40) & 0.978^{***}(\,\,\,0.12\%)(25) \\
  stars & 1.075^{**\,\,\,}(\,\,\,0.00\%)(44) & 1.058^{***}(\,\,\,0.03\%)(33) & 0.989^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.04\%)(34) \\
  project\_age & 1.066^{***}(\,\,\,0.02\%)(33) & 1.098^{***}(\,\,\,0.27\%)(17) & 1.039^{***}(\,\,\,0.14\%)(23) \\
  open\_issue\_num & 0.907^{***}(\,\,\,0.01\%)(40) & 0.995^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.00\%)(44) & 0.963^{***}(\,\,\,0.07\%)(28) \\
  open\_pr\_num & 1.711^{***}(\,\,\,3.84\%)(06) & 1.772^{***}(\,\,\,4.02\%)(07) & 1.789^{***}(\,\,\,3.82\%)(08) \\
  pr\_succ\_rate & 1.054^{***}(\,\,\,0.04\%)(29) & 1.036^{***}(\,\,\,0.08\%)(25) & 1.027^{***}(\,\,\,0.20\%)(18) \\
  pushed\_delta & 1.119^{***}(\,\,\,1.04\%)(13) & 1.128^{***}(\,\,\,2.02\%)(10) & 1.107^{***}(\,\,\,1.93\%)(11) \\
  integrator\_availability & 1.185^{***}(\,\,\,5.14\%)(04) & 1.221^{***}(\,\,\,6.81\%)(05) & 1.246^{***}(\,\,\,5.52\%)(06) \\
 \hline \\[-1.8ex] 
Observations & \multicolumn{1}{r}{116,528} & \multicolumn{1}{r}{309,649} & \multicolumn{1}{r}{1,552,437} \\ 
\hline 
\hline \\[-1.8ex] 
\multirow{2}{*}{\textit{Note:}} & \multicolumn{3}{r}{exp(coef)$^{sig}$(Sum of Square proportion)(rank)} \\
& \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table*}

==> tables/latency_diff_time_period.tex <==
\begin{table*}[!htbp] \centering
\scriptsize
  \caption{Factors influence on latency for different time period} 
  \label{latency_diff_time_period} 
\begin{tabular}{@{\extracolsep{-10pt}}lD{.}{.}{-3} D{.}{.}{-3} D{.}{.}{-3} } 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{3}{c}{\textit{Dependent variable: log(lifetime\_minutes+1)}} \\ 
\cline{2-4} 
\\[-1.8ex] & \multicolumn{1}{r}{before 2016.6} & \multicolumn{1}{r}{2016.6-2018.6} & \multicolumn{1}{r}{2018.6-2019.6}\\ 
\hline \\[-1.8ex] 
 (Intercept) & 490.176^{***} & 676.746^{***} & 813.657^{***} \\ 
    num\_commits & 1.228^{***}(\,\,\,6.36\%)(04) & 1.262^{***}(\,\,\,3.76\%)(06) & 1.322^{***}(\,\,\,2.44\%)(07) \\
  src\_churn & 1.275^{***}(\,\,\,5.34\%)(05) & 1.308^{***}(\,\,\,4.68\%)(05) & 1.310^{***}(\,\,\,3.37\%)(06) \\
  files\_added & 0.979^{***}(\,\,\,0.02\%)(31) & 0.980^{***}(\,\,\,0.03\%)(28) & 0.984^{***}(\,\,\,0.03\%)(31) \\
  files\_deleted & 0.925^{***}(\,\,\,0.98\%)(14) & 0.917^{***}(\,\,\,0.77\%)(13) & 0.916^{***}(\,\,\,0.52\%)(14) \\
  files\_changed & 1.024^{***}(\,\,\,0.00\%)(39) & 1.002^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.00\%)(39) & 0.998^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.02\%)(35) \\
  friday\_effect & 1.061^{***}(\,\,\,1.01\%)(13) & 1.068^{***}(\,\,\,0.68\%)(16) & 1.078^{***}(\,\,\,0.47\%)(15) \\
  commits\_on\_files\_touched & 0.908^{***}(\,\,\,0.66\%)(19) & 0.906^{***}(\,\,\,0.77\%)(14) & 0.916^{***}(\,\,\,0.69\%)(13) \\
  hash\_tag & 1.139^{***}(\,\,\,3.85\%)(08) & 1.174^{***}(\,\,\,3.16\%)(07) & 1.182^{***}(\,\,\,1.62\%)(10) \\
  test\_inclusion & 1.013^{***}(\,\,\,0.00\%)(40) & 0.995^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.00\%)(40) & 1.006^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.01\%)(38) \\
  description\_length & 1.422^{***}(11.41\%)(03) & 1.402^{***}(11.21\%)(03) & 1.378^{***}(10.49\%)(03) \\
  ci\_exists & 1.158^{***}(\,\,\,1.26\%)(10) & 1.223^{***}(\,\,\,1.59\%)(10) & 1.183^{***}(\,\,\,1.38\%)(11) \\
  has\_comments & 1.303^{***}(\,\,\,4.02\%)(07) & 1.233^{***}(\,\,\,2.42\%)(08) & 1.296^{***}(\,\,\,3.40\%)(05) \\
  comment\_conflict & 1.063^{***}(\,\,\,0.78\%)(16) & 1.079^{***}(\,\,\,0.89\%)(12) & 1.072^{***}(\,\,\,0.46\%)(16) \\
    num\_comments & 2.913^{***}(33.23\%)(01) & 2.662^{***}(42.09\%)(01) & 2.346^{***}(43.73\%)(01) \\
  other\_comment & 1.055^{***}(\,\,\,0.81\%)(15) & 1.035^{***}(\,\,\,0.10\%)(22) & 1.107^{***}(\,\,\,0.22\%)(18) \\
  test\_churn & 1.054^{***}(\,\,\,0.18\%)(22) & 1.061^{***}(\,\,\,0.20\%)(19) & 1.055^{***}(\,\,\,0.13\%)(23) \\
  followers & 0.939^{***}(\,\,\,0.06\%)(27) & 0.962^{***}(\,\,\,0.08\%)(24) & 1.030^{***}(\,\,\,0.19\%)(19) \\
  first\_pr & 1.017^{***}(\,\,\,0.03\%)(28) & 1.028^{***}(\,\,\,0.07\%)(25) & 1.017^{***}(\,\,\,0.03\%)(32) \\
  account\_creation\_days & 0.975^{***}(\,\,\,0.15\%)(23) & 0.972^{***}(\,\,\,0.06\%)(27) & 0.956^{***}(\,\,\,0.05\%)(29) \\
  core\_member & 0.852^{***}(\,\,\,1.22\%)(11) & 0.879^{***}(\,\,\,1.12\%)(11) & 0.876^{***}(\,\,\,1.75\%)(09) \\
  contrib\_gender & 0.986^{***}(\,\,\,0.00\%)(41) & 0.998^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.00\%)(41) & 1.004^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.02\%)(36) \\
  contrib\_open & 0.960^{***}(\,\,\,0.02\%)(32) & 0.988^{***}(\,\,\,0.01\%)(33) & 0.984^{***}(\,\,\,0.10\%)(26) \\
  contrib\_cons & 0.967^{***}(\,\,\,0.09\%)(24) & 0.954^{***}(\,\,\,0.13\%)(21) & 0.962^{***}(\,\,\,0.06\%)(28) \\
  contrib\_extra & 0.978^{***}(\,\,\,0.00\%)(42) & 0.990^{**\,\,\,}(\,\,\,0.01\%)(34) & 0.996^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.03\%)(33) \\
  contrib\_agree & 0.986^{***}(\,\,\,0.03\%)(29) & 0.990^{**\,\,\,}(\,\,\,0.01\%)(35) & 0.978^{***}(\,\,\,0.01\%)(39) \\
  contrib\_neur & 0.985^{***}(\,\,\,0.02\%)(33) & 0.989^{***}(\,\,\,0.01\%)(36) & 0.983^{***}(\,\,\,0.01\%)(40) \\
  prev\_pullreqs & 0.943^{***}(\,\,\,0.08\%)(25) & 0.980^{***}(\,\,\,0.02\%)(31) & 0.957^{***}(\,\,\,0.11\%)(24) \\
  prior\_review\_num & 1.053^{***}(\,\,\,0.02\%)(34) & 0.997^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.00\%)(42) & 0.983^{***}(\,\,\,0.15\%)(21) \\
  inte\_open & 1.097^{***}(\,\,\,0.76\%)(17) & 1.123^{***}(\,\,\,0.53\%)(17) & 1.145^{***}(\,\,\,0.33\%)(17) \\
  inte\_cons & 1.071^{***}(\,\,\,0.01\%)(36) & 1.049^{***}(\,\,\,0.09\%)(23) & 1.017^{***}(\,\,\,0.18\%)(20) \\
  inte\_extra & 0.964^{***}(\,\,\,0.01\%)(37) & 0.971^{***}(\,\,\,0.03\%)(29) & 0.983^{***}(\,\,\,0.05\%)(30) \\
  inte\_agree & 0.976^{***}(\,\,\,0.00\%)(43) & 0.992^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.00\%)(43) & 1.007^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.02\%)(37) \\
  inte\_neur & 1.031^{***}(\,\,\,0.29\%)(21) & 1.045^{***}(\,\,\,0.07\%)(26) & 1.074^{***}(\,\,\,0.03\%)(34) \\
  same\_user & 0.606^{***}(18.19\%)(02) & 0.635^{***}(16.83\%)(02) & 0.640^{***}(18.40\%)(02) \\
  sloc & 0.987^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.02\%)(35) & 0.952^{***}(\,\,\,0.03\%)(30) & 0.963^{***}(\,\,\,0.00\%)(42) \\
  team\_size & 0.908^{***}(\,\,\,0.08\%)(26) & 0.865^{***}(\,\,\,0.26\%)(18) & 0.912^{***}(\,\,\,0.14\%)(22) \\
  test\_lines\_per\_kloc & 0.990^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.03\%)(30) & 0.971^{***}(\,\,\,0.01\%)(37) & 1.042^{***}(\,\,\,0.00\%)(43) \\
  stars & 0.987^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.01\%)(38) & 0.935^{***}(\,\,\,0.02\%)(32) & 0.968^{*\,\,\,\,\,\,}(\,\,\,0.00\%)(44) \\
  project\_age & 0.925^{***}(\,\,\,0.70\%)(18) & 0.876^{***}(\,\,\,0.19\%)(20) & 0.762^{***}(\,\,\,0.11\%)(25) \\
  open\_issue\_num & 0.972^{**\,\,\,}(\,\,\,0.00\%)(44) & 0.970^{**\,\,\,}(\,\,\,0.00\%)(44) & 0.974^{\,\,\,\,\,\,\,\,\,}(\,\,\,0.01\%)(41) \\
  open\_pr\_num & 1.501^{***}(\,\,\,1.71\%)(09) & 1.798^{***}(\,\,\,2.38\%)(09) & 1.635^{***}(\,\,\,2.44\%)(08) \\
  pr\_succ\_rate & 0.973^{***}(\,\,\,0.55\%)(20) & 1.020^{***}(\,\,\,0.01\%)(38) & 1.140^{***}(\,\,\,0.07\%)(27) \\
  pushed\_delta & 1.120^{***}(\,\,\,1.04\%)(12) & 1.083^{***}(\,\,\,0.71\%)(15) & 1.094^{***}(\,\,\,1.26\%)(12) \\
  integrator\_availability & 1.249^{***}(\,\,\,4.99\%)(06) & 1.219^{***}(\,\,\,4.95\%)(04) & 1.208^{***}(\,\,\,5.45\%)(04) \\
 \hline \\[-1.8ex]
Observations & \multicolumn{1}{r}{526,220} & \multicolumn{1}{r}{848,915} & \multicolumn{1}{r}{603,479} \\ 
\hline
\hline \\[-1.8ex] 
\multirow{2}{*}{\textit{Note:}} & \multicolumn{3}{r}{exp(coef)$^{sig}$(Sum of Square proportion)(rank)} \\
& \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table*}
